Top of the Heap: Efficient Memory Error Protection of Safe Heap Objects

Heap memory errors remain a major source of software vulnerabilities. Existing memory safety defenses aim at protecting all objects, resulting in high performance cost and incomplete protection. Instead, we propose an approach that accurately identifies objects that are inexpensive to protect, and design a method to protect such objects comprehensively from all classes of memory errors. Towards this goal, we introduce the Uriah system that (1) statically identifies the heap objects whose accesses satisfy spatial and type safety, and (2) dynamically allocates such "safe" heap objects on an isolated safe heap to enforce a form of temporal safety while preserving spatial and type safety, called temporal allocated-type safety. Uriah finds 72.0% of heap allocation sites produce objects whose accesses always satisfy spatial and type safety in the SPEC CPU2006/2017 benchmarks, 5 server programs, and Firefox, which are then isolated on a safe heap using Uriah allocator to enforce temporal allocated-type safety. Uriah incurs only 2.9% and 2.6% runtime overhead, along with 9.3% and 5.4% memory overhead, on the SPEC CPU 2006 and 2017 benchmarks, while preventing exploits on all the heap memory errors in DARPA CGC binaries and 28 recent CVEs. Additionally, using existing defenses to enforce their memory safety guarantees on the unsafe heap objects significantly reduces overhead, enabling the protection of heap objects from all classes of memory errors at more practical costs.

==> 5_Design.tex <==
%auto-ignore
\section{Design}
\label{sec:design}

%\mat{Instead of talking aboust spatial, temporal, type safety one after the other, another approach would be to introduce a "type metadata store" that, per location, keeps track about its safety properties. Then introduce different analyses that refine on a per-location basis, this information so that we can then instrument accordingly in a later pass.} \kaiming{Agree, currently we changed it into this way.}

In this section, we introduce the design of the \tool.

\subsection{Overview of \tool Approach}
\label{subsec:overview}

\begin{figure*}
    \centering
    \includegraphics[width=7in]{Figures/UriahOverview.jpg}
    \vspace{-6pt}\caption{\tool System Technical Approach}
    \label{fig:arch}\vspace{-8pt}
\end{figure*}

%\trent{Problems we solve, challenges in solving, way we solve.  Start with goal of memory safe heap region.  Validate safety and challenges (solved) in spatial and type.  Allocation (runtime) goal and challenges (solved).  Focus references to dataguard to minimize.}  \kaiming{Problem: Previous efforts do not provide a solution of having comprehensive protection of safe heap objects against all classes of memory errors with low cost. Challenges are covered in Section~\ref{subsec:designbackground}}

As Definition~\ref{def:memorysafety} states, for a heap object to be safe
from memory errors, all pointers that may-alias the object (including its sub-fields) must comply with safety requirements of the heap object.  Thus, \tool
computes the pointers that may-alias a heap object and collects the unsafe operations that may result in
spatial and type memory errors associated with those pointers. If none of a heap object's pointers performs any operation that may cause a memory error (i.e., {\em statically-proven safe}, see Definition~\ref{def:staticallyprovensafe}), \tool then utilizes typed pool allocation to guarantee that the memory allocated for the said heap objects never be reused for different types of objects, which ensures the {\em temporal type safety} of the heap object. \kaiming{This paragraph goes over the high-level design of \tool, static spatial and type safe then runtime temporal type safe.}
%\trent{ensures a specific definition of temporal safety.  Finish static cases first before claims on temporal.} \kaiming{Changed to temporal type safety.}

\begin{definition}
\label{def:staticallyprovensafe}
 The term {\bf Statically-proven safe} heap objects represents the heap objects that passed the static safety validation of spatial and type memory safety.
\end{definition}

To ascertain whether a heap object is {\em statically-proven safe}, \tool employs a technique that involves identifying the types of memory errors associated with each heap object that necessitate safety validation. To accomplish this, \tool utilizes the approaches put forth by CCured (for spatial and type safety) to determine if a pointer can be used in a memory operation that has the potential to result in a particular type of memory error. The set of memory error types that must be validated for a heap object is the combination of the types that may be induced by its aliases.\kaiming{This paragraph is about the CCured analysis as our first stage analysis to find out unsafe operations - arithmetic and typecast.}

\mat{What about typing rules; those are not present in CCured.}
%\mat{Also, when introducing types, you must define what you mean for types in C and sometimes later how you disambiguate void*, char*, and struct foo* pointers as they are all interchangeable---and are often interchanged, e.g., memcpy only uses char* for arbitrary types.} \kaiming{Interpreting integer as pointer through inttoptr and ptrtoint instructions are directly identified as unsafe. Interpreting structural type to void* or char* liked behavior is considered as upcast thus is safe.}
\mat{Be explicit about these type rules somewhere, i.e., add a set of formal definitions in the design section that clarifies these questions; don't just answer me in a comment.}

For verifying the safety of the heap objects that are involved in operations that may cause spatial and/or type memory errors, \tool takes a two-step verification approach that consists of constraint collection and validation, similar to DataGuard~\cite{dataguard} System of protecting the stack. 

\tool uses the following approach to collect constraints. First, for each heap object, \tool collects constraints from the heap object's declaration for the classes of memory errors that require safety validation. These constraints are assigned to pointers whenever that heap object is assigned to a pointer (e.g., at pointer definitions) after it is allocated. For static analysis, we make such assignments based on whether the pointer may alias the heap object. Constraints are then validated on each pointer use.

%Should multiple heap objects be assigned to the same pointer (i.e., at the same pointer definition with an LLVM phi instruction), the analyses proceed independently, as these represent distinct contexts or are caught by the SSA IR form since the pointers are on the stack. State relevant to safety validation (e.g., index of a pointer in a buffer) may be updated at each pointer definition and each pointer operation (i.e., at pointer use). 

After the constraints are collected, the difficulty for constraint validation lies in maximizing the count of safe heap objects while ensuring that none of the hazardous heap objects are mistakenly classified as safe. Prior work on stack object safety, DataGuard~\cite{dataguard}, utilizes a two-stage analysis that combines static analysis and symbolic execution. We follow a similar idea in \tool framework.  
%\trent{We should describe the  approach differently in this paper.  Three steps: (1) validate spatial safety; (2) validate type safety; (3) enforce temporal safety.  Here, we should define the challenges broadly and how our design overcomes them.  E.g., heap objects are long lived, so could be hard to validate safety for all pointers.  Want to sell the big insights in the overview to get the reviewers excited.} \zhiyun{agree with Trent about bringing up the unique challenges of tracking heap objects.} \kaiming{Currently the design section follows this spirit}


%CCured identifies pointers that may cause spatial and type errors. 

For temporal memory safety, it is hard to detect safety violations based on static data flow analysis such as liveness analysis or the live-range analysis in~\cite{dataguard} using LLVM since the heap object are represented as memory locations instead of SSA variables in LLVM IR. Researchers have expressed interest in detecting potential temporal memory safety violations on the heap using static analysis, such as~\cite{uafchecker, clangstaticanalyzer, mluafdetect, gueb, uafdetector, cred,Zhai2020UBITectAP}, but we can not reuse them in our work due to the claim of unsoundness. Other works focus on eliminating temporal memory safety violations using runtime checks through dangling pointer elimination~\cite{van2017dangsan,dangnull,freesentry}, pointer dereference checking~\cite{duck2018effectivesan}, and limiting exploitability~\cite{cfixx}, which are orthogonal to our approach. Instead, \tool utilizes {\em typed pool allocation} for the {\em statically-proven safe} heap objects to ensure the {\em temporal type safety}. Theoretically, a sound static analysis that aims for identifying potential temporal safety violations such as UAF and UBI can be used to fulfill our goal of identifying temporal safe heap objects, and we leave that as our future work.
%\mat{You are describing mechanisms across the full spectrum, you likely have to break this into classes of safe/somewhat safe/unsafe/ ...} \kaiming{Yes, the per memory error classes discussion of challenges and our solutions are in the following subsections.}

\subsection{Previous efforts and Our Challenge}
\label{subsec:designbackground}

\kaiming{This is the section that we discussed to go over the previous works, list what they did, what they did not do, what are the remaining challenges for us, and how do we solve them in \tool. I tentatively use a subsection for it.}

\trent{Should be covered by the end of section 2.}\kaiming{Should we merge this subsection into Section 2? But these are design challenges that need to be solved. We can merge the description of previous work into Section 2 and reference that here, and then list the challenges here.}
For the sake of providing comprehensive protection against memory errors for heap objects, unfortunately, previous works discussed in  Section~\ref{subsec:memorysafetyforheap} are lacking in one way or another. They either aimed for a specific type of memory error, or introduced high overhead when applying a combination of them.

In \tool, the goal is to provide a comprehensive protection against memory errors for the heap objects that can be {\em statically-proven safe} (see Definition~\ref{def:staticallyprovensafe}). To accomplish that, we take advantage from several previous works, namely CCured~\cite{ccured,ccured-realworld,ccured-toplas}, SAFECode~\cite{safecode,safecode-gc}, Baggy-Bounds~\cite{baggybounds}, Type-After-Type~\cite{tat}, and DataGuard~\cite{dataguard}.

CCured~\cite{ccured,ccured-realworld,ccured-toplas} provides the definition of safe and unsafe objects for spatial and type safety, but did not contribute to temporal safety protection. For type and temporal safety of heap objects, SAFECode~\cite{safecode,safecode-gc} defines safety in
terms of points-to information, where an object is safe if it obeys
all its computed points-to relationships w.r.t. their types, and enforces automatic pool allocations of type-known objects to achieve temporal safety. However, such a solution is found to be expensive. Also, with no protection against spatial memory error, the protection can be collapsed. Baggy-Bounds~\cite{baggybounds} proposed to use value-range analysis to protect heap objects against spatial memory errors, but it is costly and spatial protection only. Type-After-Type~\cite{tat} utilizes a light-weighted design to achieve temporal type safety by introducing a new memory allocation and management scheme through typed-pool allocation, but it only enforces temporal type safety protection, remaining spatial and type errors can potentially corrupt the constructed pools. Also, they construct per-allocation-site pool that allows multiple types of objects to reside in one pool, which leaves the window for potential type unsafe memory reuse (as stated in Section~\ref{subsec:memorysafetyforheap} and~\ref{subsec:comprehensive}).



In terms of providing comprehensive memory protection, DataGuard~\cite{dataguard} examined and achieved the goal of using comprehensive and accurate static analyses to improve the scope of security and performance of runtime defenses. Inspired by a similar spirit, \tool aims for providing a comprehensive protection against memory errors for the heap objects that can be {\em statically-proven safe}. However, DataGuard was deployed for protecting stack objects, certain challenges exist of employing it on the heap, such as the more overapprixmated aliasing information, applying value-range analysis while the heap objects are no longer SSA-formed IR, and symbolic execution. Also, for temporal memory safety, it is hard to detect safety violations based on static data flow analysis such as liveness analysis or the live-range analysis in~\cite{dataguard}, since the heap object are represented as memory locations instead of SSA variables in LLVM IR, and they tend to be long-live and across multiple functions. 

\trent{problem first, then insight into how solved.} \kaiming{Yes, the following text list the challenges to achieve the goal per each step and offered high-level overview of our detailed solutions.} In \tool, the high-level design of achieving comprehensive memory error protection for heap objects is to enforce typed-pool allocation (ensuring temporal type safety) for the objects that are {\em statically-proven safe} (ensuring spatial and type safety). For all other unsafe heap objects, we isolate them to prevent the corruption of unsafe heap objects cannot harm the safe heap objects. Note that we focus on the heap objects that are referenced from the stack, heap objects that are referenced from elsewhere (e.g., global) are treated as unsafe as of now. Here, we list the challenges that need to be resolved to achieve the goal, and discuss each of them in the following sections.

\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Aliasing}}: To analyze the heap objects through references from the pointers on the stack, a sound and precise aliasing analysis are needed for classifying heap objects and applying for corresponding protection.

\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Static Spatial Safety Validation}}: Heap objects are often accessed using pointer arithmetic, so a CCured-style analysis would indicate almost all heap objects as unsafe while the truth is the majority of pointer arithmetic comes from field accesses. To fix that, \tool needs additional analyses to identify safe accesses. Previous approaches such as DataGuard~\cite{dataguard} utilized value-range analysis to validate the spatial constraints of stack objects, we have to adjust the approach to accommodate the analysis to the heap, given heap objects are represented differently as stack objects in LLVM IR and have longer live-time. \kaiming{Baggy have heap analysis, but they are not open-sourced.}

\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Static Type Safety Validation}}: Type cast serves as one of the natural of C/C++, heap objects are more involved in it. Given the fact that not all the type casts are unsafe, we need to come up with methods to validate the safe typecast statically. CCured claimed that among all type casts, 63\% are of identical types, for the remaining type casts, 93\% are safe upcast and 6\% are unsafe downcast, but did not mention specific methods for realizing such detection. EffectiveSan~\cite{duck2018effectivesan} implements an upcast check to facilitate their runtime checking, but it is only for C++, and only partially covers upcast cases, (i.e., only class inheritance). We would like to realize a type cast analysis based on that fact, to figure out the real unsafe type casts, namely downcasts and casts between incompatible types.

\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Symbolic Execution on Heap}}: Static analysis requires over-approximation to handle aliasing. We want to reduce the imprecision by strategically evaluating over-approximation. DataGuard exercised a similar idea on the stack, \tool needs to bring the methods to the heap.

\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Enforcing Temporal Type Safety}}: Type-After-Type~\cite{tat} enforced typed-pool allocation to achieve temporal type safety with the aforementioned problems. To adopt the approach for the temporal type safety, \tool needs to materialize an allocator to ensure that: (1) Heap objects allocated using per-type pool allocation scheme cannot have spatial or type memory errors. (2) The construction of pools should strictly obey per-type design, no multiple types are allowed to be in one pool. (3) Heap objects that have spatial or type memory errors should be isolated in a separate region. (4) Memory allocated for a specific type of object can only be reused later for the same type.
%\zhiyun{The per-type pool reminds me of autoslab in the Linux kernel. I remember it is a general defense against heap corruption vulnerabilities, including OOB, type confusion, and UAF. Why don't we extend the same idea to all objects? What benefits do we gain by limiting the per-type pool to only those statically-verified safe objects? Is it because it is a significant overhead to have too many per-type pools? } \kaiming{From the doc by GrSecurity (Zhenpeng Lin) of Autoslab, it is a powerful and lightweight memory management scheme that facilitates the protection of memory errors in the Linux kernel. Despite the advantages listed in the doc, it has several weaknesses related to "comprehensive" memory protection. (1) It is essentially a "per-allocation-site" pool allocation, not a per-type pool design. In most of the cases, "per-allocation-site == per-type", but it is not always true, leaving the window of placing objects of different types in one pool. (2) If we don't consider (1), saying that Autoslab enforces per-type allocation pool, it has the same security guarantee that we have - temporal type safety. (3) No protection against bad type casts. (4) AutoSlab makes overflow (spatial error) exploitation harder, but it is not fully covered. There are several scenarios discussed in the doc that shows that AutoSlab is not effective in preventing spatial error exploitations comprehensively. The per-type pool is not expensive, as examined in Type-after-type~\cite{tat}, but it does not provide spatial and type protection, for spatial, at least the in-pool overflow is allowed, similar to AutoSlab. }




\subsection{Pointer Alias Analysis of Heap Objects}
\label{subsec:alias}
\trent{This is the sound alias analysis section, right?  Sound analysis in general section to be done?} \kaiming{This is the section for we to illustrate the alias analysis that we used and its soundness. Previously we discussed to attach the soundness argument into each corresponding subsections.} \tool's safety validation methods require finding all pointers that may-alias each heap object. For that,  \tool leverages context-sensitive pointer alias analysis on the heap by combining the SVF pointer alias analysis~\cite{svf,sui2012issta,sui2014tse,sui2016fse,sui2018tse} intraprocedurally based on its VFG and the PDG representation
of PtrSplit~\cite{Liu17CCS} to represent the data flows between
functions to compute interprocedural may-aliases. 
\begin{comment}
\zhiyun{My understanding is that SVF's pointer analysis is not sound. It can also be very imprecise when analyzing programs with multiple entry points (syscalls or any program that takes multiple rounds of inputs). That's why we developed our own pointer analysis that is much more precise, specifically for multi-entry programs: ``Statically Discovering High-Order Taint Style Vulnerabilities in OS Kernels, CCS 2021''. Probably can cite it and discuss it.} \kaiming{Our pointer alias analysis is not solely based on the SVF pointer alias analysis but is a combination of PDG and SVF. PDG utilizes SVF internally and has already demonstrated its soundness. The soundness of SVF individually, however, is not formally proved in their paper, but we identified that it satisfied the requirements of being sound when dealing with heap objects from a set of papers~\cite{svf,sui2012issta,sui2014tse,sui2016fse,sui2018tse}. Theoretically, SVF is sound for aliasing of the scenario of stack pointers to heap objects. However, implementation-wise, there could be issues that render it to be unsound, which is related to the relative-soundness that we discussed in DataGuard~\cite{dataguard}. Another important reason for us to pick SVF is that it is used in PDG implementation and is compatible with the toolchain. Thanks for the pointer to the paper, I will discuss it in the last paragraph of this subsection.} 
\zhiyun{Thanks for the clarification. I understand your argument that it is by design sound. However, what I am trying to say is that it is, by design, not sound. In fact, any flow-sensitive pointer analysis is, by design, not sound when analyzing multi-entry programs.
To understand this, consider two entry points 1 and 2, we need to consider the results when entry1() is executed before entry2() and vice versa. We also need to consider different sequences of entry1() and entry2() invocations, e.g., 1-2-1-2-1-1-2, to converge to a fixed point. When there are many entry points, it becomes impractical to enumerate all possible sequences of entry-point invocations. My understanding is that SVF tries to be flow-sensitive but it does not really handle multi-entry applications at all (it assumes a single entry only). Also, nginx, httpd, proftpd, and opensshd are can be viewed as multi-entry programs because they essentially run with a giant loop that processes multiple types of requests (each type of request handler can be considered a different entry point). A sound flow-sensitive pointer analysis will need to analyze multiple loop iterations and converge to a fixed point. That said, if you really want to claim design-level soundness, I think we can potentially configure SVF to perform a flow-insensitive pointer analysis, which by design will over-approximate things.} \kaiming{Thanks for pointing the issue out, we were actually not aware of this issue previously. To me "enumerating different sequences entry to examine possible execution sequences or reach a fixed point" is more like a path-sensitivity issue, and in our work, we already run it in a path-insensitive way, that is the reason why our static analysis often overapproximate unsafe operations and need symbolic execution. Also, a key measure of whether an alias analysis work handles heap soundly is whether it handles heap cloning soundly, SVF did so-called lazy heap-cloning but it is still sound. We use SVF for the intra-procedural alias analysis and use PDG to bridge it to inter-procedural in a context-sensitive way. As I mentioned in the last paragraph of this subsection, we probably discuss it in the discussion or related work.}
\zhiyun{I disagree with your assessment that this SVF is sound when analyzing multi-entry programs (I actually talked to the author of SVF, i.e., Prof. Sui, and he agreed that SVF is not designed to handle multi-entry programs so it won't be sound by design). This is a complicated issue and we have actually written a paper on how to perform a sound alias analysis for multi-entry programs (under submission). The first step we took is to give up flow-sensitivity (and I believe SVF is by design flow-sensitivity). Anyway, I agree perhaps the best we can do now is to just acknowledge this issue and discuss it in the discussion section. } \kaiming{Thanks for the clarification and sorry for the confusion by my reply, I actually was not trying to argue that SVF is sound for the multi-entry programs. Again, actually, we were not aware of this issue previously, we identified that SVF did not provide the proof of its soundness formally, proposed and discussed by~\cite{javaheapcloningase,javaheapcloningpldi,Lattner2007MakingCP} , the sound handling of heap cloning is the judgment of whether a heap alias analysis is sound, and we found SVF qualify this requirement from a set of their paper. I guess the major problem seems to be that only requiring sound heap cloning is not enough. It is exciting to know that you already discussed with Prof. Sui about this issue and made improvement to it. In my previous comment-reply, I wanted to say that we only used “pure SVF”  for the intra-procedural alias analysis (is this still a problem for intra-procedural SVF?) and additionally used PDG - which contains a module named parameter-tree, for handling the aliasing queries inter-procedurally - given they already claimed soundness in the PtrSplit paper~\cite{Liu17CCS} “PtrSplit uses a PDG representation that soundly represents pointer data as parameter trees, and tracks pointer bounds for automatic marshaling and unmarshalling without user involvement.”. Also, one of the reasons that we picked SVF is that PDG also used SVF internally so it is compatible with our toolchain. But, might the case that the PDG also did not handle the multi-entry program soundly, I will check with the guy who currently maintains the PDG framework. I agree with your suggestion that we definitely need to discuss this problem in this paper for the soundness concern. At a high level, we are trying to express this paper in a way similar to DataGuard, where a combination of static analysis and runtime enforcement can be utilized to achieve comprehensive protection of heap objects that are verified as memory safe, that said, my opinion is that this problem can also be discussed in the context of relative-soundness.}
\zhiyun{sounds reasonable to me. My understanding is that no alias analysis (if it is flow-sensitive by design) can claim soundness when handling multi-entry programs. I don't think heap cloning or intra-procedural analysis would change anything.}
\zhiyun{I talked to my student working on the sound alias analysis on this. Here is what he said: I agree that flow-sensitive analysis are by design not sound with multi-entry programs. There is Andersen in SVF, which is flow-insensitive by default (which have a chance to be sound against multi-entry programs). However, it depends on the graph that Andersen is applied on. If it is on StaticValueFlowGraph (SVFG), since the graph is flow-sensitive, the analysis will not be sound. If it is performed on PAG (which is not flow-sensitive), it can have a chance to be sound.}\kaiming{Thanks for making the clarification and the input, I will investigate and probably make adjustments to \tool if needed. Definitely, this is something that we would want to discuss in the paper.}
\zhiyun{one more comment from my student: ``And I think heap cloning or the PDG strategy is about context-sensitive (making the analysis more precise), which doesn’t matter to soundness.''} \kaiming{Yes, heap cloning is about context-sensitive, as I mentioned in the next paragraph, "Heap-cloning is proposed in 2004 for facilitating dynamic symbolic execution and context-sensitive heap pointer alias analysis on Java~\cite{javaheapcloningase,javaheapcloningpldi} and has been brought into C/C++ for facilitating the sound context-sensitive heap pointer alias analysis in 2007~\cite{Lattner2007MakingCP}". Alias analyses that aimed to be sound and context-sensitive need to handle heap cloning in a sound way, as discussed in both Sea-DSA~\cite{sea-dsa} and SVF~\cite{Barbar2020FlowSensitiveTH}. Actually the second paper~\cite{Barbar2020FlowSensitiveTH} discussed about combining heap cloning with the flow-sensitive alias analysis and its soundness, and that is the reason why we said it is sound previously as they did not mention the issue that we discussed above. I'm not sure what you mean by "PDG strategy", but the PDG framework introduced by PtrSplit paper~\cite{Liu17CCS} is a sound and context-sensitive pointer alias analysis framework.}
\end{comment}

SVF heap alias analysis realizes context-sensitive alias analysis on the heap by utilizing the method called {\em Heap-Cloning} soundly. Heap-cloning is proposed in 2004 for facilitating dynamic symbolic execution and context-sensitive heap pointer alias analysis on Java~\cite{javaheapcloningase,javaheapcloningpldi} and has been brought into C/C++ for facilitating the sound context-sensitive heap pointer alias analysis in 2007~\cite{Lattner2007MakingCP}. Heap cloning distinguishes heap objects by (acyclic) call paths, creating copies at the object level, not just by allocation site. Heap cloning is essential because it allows analyses to distinguish different instances of a logical data structure created at different places in a program, even if the data structure is implemented with a common set of functions (e.g., a data structure library) that allocate memory internally. 

While the Heap-cloning technique itself is sound, SVF aims to perform {\em lazy} Heap-cloning by incorporating lightweight type information within standard flow-sensitive pointer analysis when applicable~\cite{Barbar2020FlowSensitiveTH}. When an untyped heap object is allocated at a certain point in a program, it can be replaced with a new, uniquely identified object of a specific type, and creates clones based on the type information available at the relevant points in the program. This approach is more efficient since it lazily creates typed objects only at the type initialization points where the object's type is assigned. To retain soundness, SVF requires the program to obey the {\em strict alias rule}, which means dereferencing pointers to objects of different types will never refer to the same memory location. Since our typed-pool allocator based on TCMalloc already guarantees this \trent{Can we assert this requirement up front (for static analysis) and then ensure its enforcement when we discuss runtime.} \kaiming{Yes, we can do it in that way.}, \tool leverages SVF's heap alias analysis in a sound way. Additionally, given the PDG representation is claimed to be sound as well, \tool soundly overapproximates the set of pointers that may alias a heap object.


\subsection{Spatial Safety}
\label{subsec:spatial}

CCured shows that pointers used in pointer
arithmetic operations (called sequential or {\em seq} pointers by
CCured), such as accessing array elements or structure fields, may
cause spatial memory errors. While CCured requires runtime checks for
such pointers, \tool labels any objects that may be referenced by such
pointers as requiring validation for the spatial error class. Note that \tool treats fields within compound objects, including buffers, as distinct variables since they are referenced by pointers from the stack, similar to the methodology used in~\cite{dataguard}. The difference is that once there is a field is validated as unsafe, the entire heap object is then classified as unsafe as well. \trent{Why is this OK for the stack and not for the heap?  What problem does the heap present?  Be careful stating a negative property of DG.} 

\kaiming{There is no downside of DG that forces us to do in this way on the heap. For the stack, once we identified a field to be unsafe, we place that field on the unsafe stack and redirect all references to that field to the unsafe stack. This is trivial for DG since all fields are treated as distinct variables if they are on the stack and in SSA form, in this way, the corruption of the unsafe field does not harm other safe fields.}

\kaiming{However, for the heap, it is impossible to do so since heap objects are not in SSA form. Sub-fields of Heap objects can be accessed and validated "as distinct variables" in the static analyses since they are accessed by pointers on the stack. But the runtime isolation cannot be done in this way as similar to DG. We have to say a heap object is unsafe if we identify at least 1 sub-field is unsafe in the static analyses phase to facilitate the runtime allocation/isolation. It is impossible (or might be possible but definitely much harder) to do it similarly to DG in an IR/compiler/allocator-level solution since heap objects are not in SSA. Plus, it could harm the typed pool allocation for the safe region and leave threats to the safe objects. }

\subsubsection{Spatial Constraints}
\label{subsubsec:spatialconstraints}
As is typical since the CCured
method was proposed~\cite{ccured}, checking spatial safety involves
determining the size of the object and ensuring that all accesses are
within the bounds determined by that size.  To check such a
requirement statically, ~\cite{dataguard} proposed spatial constraints for the stack objects. For adapting the similar idea to the heap, we require the following information. Heap
objects that do not satisfy the constraints defined in Table~\ref{tab:spatialconstraint} will be conservatively classified as unsafe heap objects.  \trent{Anything new from DG?  What about field of heap object issue from above?} \kaiming{In DG we extract constraints from the objects directly, but in \tool we have to extract constraints through allocation functions.}
\begin{comment}
\trent{"following four constraints"?  I assume you mean Table 1.  Are these any different than for DataGuard?  If not, we should focus on heap issues.} \kaiming{Yeah I meant Table 1, forgot to change the text after I put the constraint definition to table.}

\kaiming{For spatial safety validation, the major difference between Uriah and DataGuard lies in how do we collect the spatial constraints w.r.t. the definition and access of a heap objects. In DataGuard, such constraints can be directly extracted from IR. In Uriah, since heap objects are not modeled as SSA variables in IR, such information is missing. We have to (1) extract those from memory allocation functions (such as malloc) for the size constraints (described in Table 1) upon allocation (In DataGuard, the size constraints is directly available in IR), and (2) extract the access range of heap objects upon use by leveraging the pointer aliasing analysis for pointers from stack to heap (PDG and SVF) (In DataGuard, we are able to use points-to analysis to extract access range since both pointer and stack objects are SSA, now we have to use the more overapproximated one – aliasing analysis since heap objects are no longer SSA).}
\end{comment}
\begin{comment}
\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Declaration}}: The {\em size} from the object's {\em base}
  must be declared as a constant value through allocation function such as malloc.  The initial {\em index} is 0.

\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Definition}}: When a pointer is
defined to reference the object, the reference may be {\em offset}
to change the index.  This offset must be a constant value.

\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Use}}: When a pointer is used in an
operation, the pointer may be further offset to change the index.  Each offset in a use must also be a constant value.

\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Validation}}: For all uses, pointer {\em index} 
  $<$ {\em size} and {\em index} $\geq 0$\vspace{0.01in}.
\end{comment}


\begin{table}[ht]
    \centering
	\small
	\begin{tabularx}{8.5cm}{c|X}
	    \toprule
		\multicolumn{2}{c}{\bf\em Spatial Constraints}\\
		\midrule
		{\bf\em Declaration}&The {\em size} from the object's {\em base}
  must be declared as a constant value through allocation functions such as malloc.  The initial {\em index} is 0.\\
	    \midrule
		{\bf\em Definition}& When a pointer is
defined to reference the object, the reference may be {\em offset}
to change the index.  This offset must be a constant value.\\
		\midrule
		{\bf\em Use}&When a pointer is used in an
operation, the pointer may be further offset to change the index.  Each offset in a use must also be a constant value.\\
		\midrule
		{\bf\em Validation}&For all uses, pointer {\em index} 
  $<$ {\em size} and {\em index} $\geq 0$\\
		
		\bottomrule
	\end{tabularx}
        \vspace{0.05in}
	\caption{Processing Spatial Safety Constraints}

	\label{tab:spatialconstraint}
\end{table}

  



To check that a heap object is free of spatial errors, the heap
object must be declared with constant size when allocated. An index of the pointer into the heap object is maintained as metadata for following validation. Pointer definitions and uses may only change the value of the index by a constant offset.  The resultant index from the combination of offsets in pointer definitions and uses must be within the range of the heap object on each use, i.e., greater than 0 and less than the object size.


\subsubsection{Validating Spatial Safety}
\label{subsubsec:spatialvalidate} 
Spatial safety analysis is
performed using static analysis to classify pointers to
find pointers that may be proven safe, similarly to the Baggy Bounds~\cite{baggybounds} and SAFECode~\cite{dhurjati_dsn06,safecode-boundscheck} optimizations. \tool first performs a {\em def-use
  analysis}~\cite{LLVM-def-use} on each pointer detected (i.e., seq pointers by CCured's definition and its aliases) to
require spatial safety validation.  
%\trent{"pointer detected"?  Aliasing?  Need to specify this.} \kaiming{Seq pointers from CCured and their aliases} 
LLVM uses SSA form for its
intermediate representation, so each pointer has only one definition,
but may have many uses. To assess
bounds statically, \tool performs a {\em value range
  analysis}~\cite{value-range-book,Douglas11SBLP,dataguard} for
each pointer use from its definition, similar to ~\cite{dataguard}. Value range analysis is a type
of data-flow analysis that tracks the range (interval) of values that
a numeric variable can assume at each point of a program's execution.  \trent{Nothing new to here, I presume.  Should be summarized very briefly.}
To validate spatial safety for all possible program executions, every pointer that may alias the heap object must use offsets from the object's base whose
value range is between 0 and heap object size as determined by the
spatial safety constraints. Note that When applying value-range analysis on the heap, turns out that we need to have more heap objects to verify (more aliases) and longer data flow (def-use chain) to examine (long-liveness), these would lead to even more memory consumption compared to the stack.
 
To solve this problem, we came up with the approach – flexible context-sensitivity of value range analysis, instead of doing full context-sensitive analysis. \trent{Does Baggy mention context-sensitivity?} \kaiming{No} The goal is instead of verifying constraints in a fully context-sensitive manner, we cut off at a certain call depth to reserve a reasonable memory consumption.  \trent{I thought we use "call-strings" approach.  Using something ad hoc when there is a well-known solution is not desirable.   If we used call-strings to achieve this goal, we should say that.} \kaiming{No, we did not use call string but used context-sensitivity level.} Soundness is still retained in this approach as we classify any validation that requires exploring beyond the pre-set context-sensitivity level as unsafe.  \trent{Please integrate the symbolic execution section with this section.} \kaiming{But symbolic execution is also used for type safety validation, should we split SE into these 2 sections, spatial and type? We discussed previously to write static analyses and SE independently though.}
\begin{comment}
\trent{Symbolic?  Is there anything new here relative to DataGuard?  Nothing obvious that I see.  Question I would have is why is the stack analysis of DataGaurd appropriate to heap objects (or not).  Was there any change?  Why necessary and why works?} \kaiming{This is not for SymExec, but for VR. Apart from the differences that I listed in the previous comments, another difference here is that due to the long-living attribute of heap object, and the aliasing analysis for heap is largely overapproximated than stack to keep soundness, the analyses in Uriah are more over-approximated that the stack analysis, which result in more unsafe heap objects comparing to DataGuard.}
\end{comment}

\subsubsection{Spatial Safety Validation Soundness}
\label{subsubsec:spatialsound} 

\trent{Best to collect all these soundness statements in one place at the end.} \kaiming{One soundness subsection in the end for all the methods that we used?} Multiple prior static analyses form the basis of safety validation's static analysis methods. These include LLVM's def-use analysis, SVF pointer alias analysis using its VFG~\cite{svf,sui2012issta,sui2014tse,sui2016fse,sui2018tse}, Program Dependence Graph of PtrSplit~\cite{Liu17CCS}, and value range analysis~\cite{value-range-book,Douglas11SBLP,dataguard}. While these analyses are claimed to be sound in their respective papers, their soundness arguments are mostly informal, with the exception of value range analysis~\cite{value-range-book}. Therefore, there is a possibility that these analyses and their implementations may not cover all corner cases in sound ways. To address this, \tool relies on {\em relative soundness} - assuming the prior analyses are sound, \tool's static analyses achieve soundness. This separation of analyses in \tool{} from their application allows for a more robust and effective approach to safety validation with over-approximation.

Value range analysis~\cite{value-range-book,Douglas11SBLP,baggybounds,dataguard} is utilized in spatial safety validations to determine the potential index ranges when accessing heap objects. The analysis is performed through the PDG and only tracks simple patterns such as pointers with constant offsets from heap object bases and constant offsets when dereferencing pointers, with the constraints assigned on pointer declarations and/or definitions to a heap object with concrete size through memory allocation function. Since the PDG is deemed sound and all constants are assumed (Section~\ref{subsec:assumptions}) to be stored in read-only memory without being copied into read-write memory~\cite{ge17ndss}, it is evident that \tool's value range analysis is also sound.

\subsection{Type Safety}
\label{subsec:type}

CCured shows that pointers used in type-casting operations may
cause type errors, but we find that the majority of them can be verified as safe.  The challenge is to identify the safe cases among all type casts, as stated in Section~\ref{subsec:memorysafetyforheap} and~\ref{subsec:designbackground}. 
\trent{CCured and DataGuard are the only two?  Everyone probably relies on CCured checks to enforce type cases at runtime.} \kaiming{We don't rely on other though, and we have additional checking for the compatible type cast.} Dataguard~\cite{dataguard} did the first try but only for integer stack variables. To expand on top of that, \tool labels objects that may be referenced by such pointers as requiring validation for the type error class. Note that LLVM casts unions into structures or primitive types, and it occasionally uses {\em ptrtoint} and {\em inttoptr} cast instructions for accessing fields of compound objects; so such cases are identified by \tool as requiring type safety validation.
\begin{comment}
\mat{What about unions? Typedefs?} \kaiming{Good point, unions are cast into structures or primitive types in LLVM naturally, typedefs are treated as normal types as long as the type information is available, otherwise we directly say it is unsafe.}
\end{comment}

\subsubsection{Type Constraints}
\label{subsubsec:typeconstraints}

\tool focuses on validating the safety of integer and structural type casts.
%, particularly aiming to validate
%when signed-unsigned casts are safe for use in bounds checking.
Below, we describe the requirements for type safety validation for
heap objects and the definition and use of their references in Table~\ref{tab:typeconstraint}. \kaiming{Note that dynamic allocation of heap objects allows allocation sites to allocate objects of different types and sizes, i.e., dynamically typed allocation. Previous works~\cite{tdi, tat} utilizes the hash value of the callsite to represent the "type" of such allocations instead of the actual type of objects.  We do not reuse that scheme in \tool, instead, we say the objects that do not have type information available statically are directly classified as unsafe.}\trent{Good point to include.  Why are type safety enforcement systems not useful for us?  Like baggy eliminates safe cases with VR?  I guess type safety enforcement works from CCured's safety validation.} \kaiming{It is not "type safety enforcement systems not useful for us", it is their way to "deal with dynamically-typed heap objects" is not useful for us. Upon such case, previous approaches used "call site" as the substitution of their "type" to make their life easier. However, if we do it in the same way - mark callsite as type, we will end up with putting multiple types of objects in one pool.}


\begin{comment}
\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Declaration}}: Heap objects are
assigned the {\em type} and {\em value} (optionally only for integer variables) used in the declaration through allocation functions such as malloc. 
  
\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Definition}}: When a pointer is
defined to reference the heap object, if the operation includes a type cast
the {\em newtype} is identified. The {\em newtype} is recorded with the original {\em type} for validation. If validation succeeds {\em type} is
assigned to the {\em newtype}.  

\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Use}}: When a pointer is used to
reference the object, if the operation includes a type cast the {\em
  newtype} is identified.  The {\em newtype} is recorded with the original {\em type} for validation. If validation succeeds {\em type} is
assigned to the {\em newtype}.  If the operation assigns a 
  value, the {\em value} is stored.

\vspace{0.02in}
\noindent$\bullet$~\textbf{\textit{Validation}}: For a definition or
use that produces a {\em newtype}, we utilize additional static analysis to check whether {\em newtype} and {\em type} are {\em compatible} types. For integer variables, we require the resultant type cast
  must not change the {\em value} of the integer object referenced (e.g., by
  changing size or signedness).
\end{comment}

\begin{table}[ht]
    \centering
	\small
	\begin{tabularx}{8.5cm}{c|X}
	    \toprule
		\multicolumn{2}{c}{\bf\em Type Constraints}\\
		\midrule
		{\bf\em Declaration}&Heap objects are
assigned the {\em type} and {\em value} (optionally only for integer variables) used in the declaration through allocation functions such as malloc. \\
	    \midrule
		{\bf\em Definition}& When a pointer is
defined to reference the heap object, if the operation includes a type cast
the {\em newtype} is identified. The {\em newtype} is recorded with the original {\em type}. If validation succeeds {\em type} is
assigned to the {\em newtype}.  \\
		\midrule
		{\bf\em Use}&When a pointer is used to
reference the object, if the operation includes a type cast the {\em
  newtype} is identified.  The {\em newtype} is recorded with the original {\em type} for validation. If validation succeeds {\em type} is
assigned to the {\em newtype}.  If the operation assigns a 
  value, the {\em value} is stored.\\
		\midrule
		{\bf\em Validation}& For a definition or
use that produces a {\em newtype}, we utilize additional static analysis to check whether {\em newtype} and {\em type} are {\em compatible} types. For integer variables, we require the resultant type cast
  must not change the {\em value} of the integer object referenced.\\	
		\bottomrule
	\end{tabularx}
            \vspace{0.05in}
	\caption{Processing Type Safety Constraints}
    \vspace{-0.2in}
	\label{tab:typeconstraint}
\end{table}
  


For type safety validation, we require the object must only be cast into the {\em Compatible} types of its original type, and integer type casts must not change the value associated with the reference to change. \trent{is type compatibility defined somewhere explicitly?  Does this differ from type safety in temporal type safety?} \kaiming{Yes, see Definition~\ref{def:compatibletype}.}This check enables validation of safety from unsafe downcast and integer overflows. Also, the collected type metadata of the heap objects will be used for the typed pool allocation - to ensure temporal type safety by instrumenting the allocator.  

\begin{comment}
\trent{integer type constraints defined in DataGuard, right?  Upcasts for compatibility was first proposed by CCured?  Any issues with heap analysis for safety?} \kaiming{Yes, integer from DataGuard with the extension to track the integer serves as the bounds or access range of heap objects through alias analysis. Upcast was treated as safe in CCured, the definition of compatible type are provided by us and that includes upcast. Also, CCured did not release implementation and the work - Nescheck that we used, did not contain the upcast analysis.} \kaiming{For the issue with heap analysis for type safety, please see the comments that I added above Definition 4.}
\end{comment}

\subsubsection{Validating Type Safety}
\label{subsubsec:typevalidate} 

For integer variables, since validating type safety involves checking that values do not change on type casts, the core of type safety validation of integer variables is in the static value range analysis.  If a heap object that is validated for type safety is also used as a bound or memory (e.g., array) index, \tool uses the result of type safety to validate spatial safety (i.e., all such integers must be safe from type errors).  \trent{ideally, a type cast preserves the value.  Value has to be above X to cause that.  Can check value range.  Drop the discussion of bounds, since that has already been checked.}

For structural heap objects, the challenge is to assess whether {\em newtype} and {\em type} are compatible types. Based on Definition~\ref{def:compatibletype}, we claim that the cast from {\em type} to {\em newtype} must be either (1) cast between equivalent types, or (2) upcast. The identification of (1) is straightforward, we mainly focus on discussing our methods for (2) below.

\begin{figure}[t]
\centerline{\includegraphics[width=2.3in]{Figures/upcast1.png}}
\caption{1st Scenario of Upcast.}
\label{fig:upcast1}
\end{figure}

\begin{figure}[t]
\centerline{\includegraphics[width=2.3in]{Figures/upcast2.png}}
\caption{2nd Scenario of Upcast.}
\label{fig:upcast2}
\end{figure}

\begin{comment}
\begin{figure}
  \begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.35]{Figures/upcast1.png}
    \caption{1st Scenario of Upcast}
    \label{fig:upcast1}
  \end{minipage}%
  \begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.35]{Figures/upcast2.png}
    \caption{2nd Scenario of Upcast}
    \label{fig:upcast2}
  \end{minipage}
\end{figure}
\end{comment}




Based on our investigation, the upcasts between two structural \trent{structured} types always fall into two categories. The first one, as shown in Figure~\ref{fig:upcast1}, shows the scenario that one type (i.e., tiny\_t) serves as a field in another type (i.e., huge\_t). The second one, as shown in Figure~\ref{fig:upcast2}, shows the scenario that all fields of one type (i.e., tiny\_t) are also declared to be the fields of another type (i.e., huge\_t) with respect to their original order and starts from the base offset 0. For retaining soundness, we say any other cases of type casting that do not comply with the two scenarios above are not upcasts.


To identify the first scenario, we check for all cast instructions, whether the first field of {\em type} (recursively) is of the same type of {\em newtype}. For the second scenario, we check for all cast instructions, assuming {\em newtype} has {\em n} fields, whether the first 1 to n fields of {\em type} matches all the fields in {\em newtype} with respect to the order and sequence. Note that~\cite{ccured,ccured-realworld,ccured-toplas} claims that among all type casts, 63\% are of identical types, for the remaining type casts, 93\% are safe upcast and 6\% are unsafe downcast, based on this knowledge, we argue that this approach makes huge improvements on top of previous methods.

\begin{comment}
\mat{At this stage the policy should be clear along with its intentions/effects. So far, the text is too vague and the policy is not defined with sufficient detail.}
\mat{Before going into how you achieve it (starting next subsection), make sure the policy is crystal clear.}
\mat{Say that your static analysis groups objects into different classes (as you're later referring to these classes without introducing them here)} \kaiming{My sense is the detailed description about the classification policy is given in the text above, but turns out the reader might get drown into the text, we will need to name the unsafe objects find by Uriah, such as Uriah-seq and Uriah-wild to make it clear to readers.}\trent{We need to clear about what must be done (policy), what the challenges are and our insight, and then address the challenges one-by-one.  We need to credit other work that we are building on - erring on over-credit.}  
\end{comment}

\subsubsection{Type Safety Validation Soundness}
\label{subsubsec:typesound} 

\tool validates the type safety of heap objects for two cases: (1) \tool classifies the type casts on integer objects that never change their value as safe~\cite{dataguard}, which relies on the value range analysis that has already been proven sound~\cite{value-range-book} and (2) \tool classifies compatible type casts on objects of structured types as safe. As illustrated in Section~\ref{subsec:type}, our compatible type cast identification method is built on top of the definition of upcast in CCured~\cite{ccured,ccured-realworld,ccured-toplas}, which is demonstrated as sound. 
%Though our current methods of identifying upcast may not be complete (i.e., may have false negatives), w
We classify any heap objects that do not pass the safety validation as unsafe, which means we do not mis-classify any unsafe heap objects as safe. Thus, \tool overapproximates the unsafe type casts of heap objects in the program to retain soundness.

\subsection{Symbolic Execution Validation}
\label{subsec:symexec}
Static analysis requires over-approximation to handle aliasing. We want to reduce the imprecision by strategically evaluating over-approximation. One issue with the findings of static analysis is that they may flag certain cases as unsafe which could be false positives resulting from the inherent overapproximations of the sound analysis. Given heap alias information is more overapproximated than stack~\cite{dataguard}, heap objects are more likely to be classified as unsafe due to overapproximated aliasing. In order to address this, \tool incorporates guided symbolic execution to verify whether any of the positives identified during static analysis can be proven safe. To do this, \tool symbolically executes the part of the program
covered by the def-use chains of each pointer that may alias the heap
object, starting from the allocation of the heap object, similar to the approach adopted in~\cite{dataguard,Zhai2020UBITectAP,increlux}. 
\begin{comment}
\trent{What is the policy of a safe object wrt symbolic execution?  This also sounds similar to DataGuard.} \kaiming{Symbolic execution in \tool aims to find out the false-positive cases classified as unsafe in static analysis phase due to over-approximation, thus, it validates from the allocation of the heap objects to the unsafe access, to see whether that is feasible during actual runtime, which follows the similar idea of DataGuard.}
\zhiyun{The principle does sound similar to DataGuard. Maybe we can give a citation. This strategy is actually used in UBITect and IncreLux as well (Yizhuo's work). Wondering if it makes to cite also.} \kaiming{Cited.}
\end{comment}

\subsubsection{Applying Symbolic Execution}
\label{subsubsec:applyse}
\trent{This is a good section.  Should elaborate on the pruning of illegal paths vs validation of safe operation.  And why that is sufficient.  Still like to see this integrated with spatial and type analyses rather than separate.} Symbolic execution depends on the results of static analyses, if static analyses identifies a heap object as unsafe, it means that the object either violates constraints or aliased by unsafe objects/pointers. We've observed that the lack of path sensitivity and overapproximation of alias in the analysis can result in imprecision and false positives, as the effects of multiple program branches or unrealistic aliasing may inaccurately indicate that the object is unsafe. Symbolic execution can address this by assessing these paths independently and examining the def-use chain independently per unsafe cases.

When performing type safety validation, if compatible-type-cast analysis identifies a heap object as unsafe, it is usually because of either an incompatible type cast or missing type information during static analysis. In the former case, \tool uses symbolic execution from the allocation of the heap object to the type cast instruction that triggers the alarm. This approach helps to verify whether it is a true positive. %\trent{Meaning unsafe.  Try to be direct.}


%Copied from DataGuard paper
A challenge in using symbolic execution is to avoid path explosion.
Since \tool employs symbolic execution on the positive (i.e., presumed
unsafe) cases found by static analysis, we only need to symbolically
execute the program from the allocation of heap objects to its last
unsafe use in its def-use chains, through pointers, which improves \tool's ability to
identify safe cases over pure symbolic execution without static
analysis.  \tool applies LLVM’s loop
simplify and canonicalization
technique to reduce the path
explosion problem introduced by loops, as applied in patch generation
to satisfy safety properties~\cite{huang19oakland}. \tool also
leverages symbolic state merging employed by S2E~\cite{s2e} to
eliminate unnecessary forks when encountering branches, which reduces
the number of paths to explore by orders of
magnitude~\cite{s2e-state-merging}.  To avoid path explosion in long
sequences of def-use chains, we limit the analysis depth.  As
longer def-use chains are more likely to lead to unsafe operations, we
focus on shorter paths.  
%\trent{Also overlap from DataGuard.}

\subsubsection{Symbolic Execution Soundness}
\label{subsubsec:sesound}

First, path explosion in symbolic execution often means that it is
impractical to execute all paths in the program, even with loop canonicalization and symbolic state merging. \tool limits the
depth of the symbolic execution to avoid expensive cases, but any
symbolic execution terminated for this reason classifies the
associated heap object as unsafe. Second, symbolic analyses may sacrifice soundness when employing
concrete values for some variables, creating a concolic
execution~\cite{SurveySymExec-CSUR18, s2e}.  \tool only concretizes
values that are constants in spatial safety analysis.  All other variables
are initialized with symbolic values.  Only
symbolic values are used to initialize variables in the temporal
analysis. Third, \tool's symbolic executions utilize the def-use chains soundly
in validating heap objects found unsafe by static analysis.  The
symbolic execution analysis starts at the allocation of heap objects
and symbolically executes the program until the last unsafe pointer
operation (use) of any alias of the heap object. Thus, all
paths that can possibly lead to a memory error are executed
symbolically before a heap object can be declared safe.
 \tool only allows safe objects (i.e., proven by the
  static analysis) to be used in any constraints derived from the
  symbolic execution.  Unsafe objects remain symbolic, so they are not
  constrained during the execution.  The loop-canonicalization
applied to simplify loops~\cite{huang19oakland} and symbolic state
merging~\cite{s2e-state-merging} are also sound.


\subsection{Temporal Safety}
\label{subsec:temporal}

\subsubsection{Temporal Safety Overview}
\label{subsubsec:temporaloverview}
As described in Section~\ref{subsec:overview}, for temporal memory safety of heap objects, it is hard to detect safety violations purely relying on static validation. Given that temporal errors, unlike spatial and type errors that can be resolved by leveraging static safety validation, are more difficult to prevent. To fully protect against them, we would need to monitor every pointer in memory which results in high overheads~\cite{van2017dangsan,dangnull,caver,safecode,freesentry,safecode-gc}. Given the truth that temporal exploitation usually involves reacquiring the memory of different types of objects, enforcing type-safe memory reuse (i.e., temporal type safety, see Definition~\ref{def:temporalsafety}) is a more practical solution~\cite{cling,tat,tdi} to mitigating temporal errors with lower overhead as defined below. \trent{Past work enforces this one.  Ideally, would have defined temporal type safety by now.} \kaiming{My opinion is that we need to put all definitions as earlier as possible and reference them when need. Take this as an example, we will also need to mention temporal type safety in earlier sections, putting definition at here would lead to confusion I guess.}



Though temporal type safety does not entirely prevent attackers' reuse-based memory accesses, it does, however, constrain the attacker by ensuring that any access is type-safe.  Unfortunately, current methods for implementing type-safe memory reuse are less efficient and accurate because they determine allocation types at runtime~\cite{cling}. Some researchers have utilized static type identification~\cite{tat,tdi} to guide the type-safe memory allocation and reuse type-specific regions for lower overhead, but they used allocation sites instead of types for dynamically-typed objects. \trent{problem} However, dynamic allocation of heap objects allows allocation sites to allocate objects of multiple types and sizes. Consequently, their method may permit the reuse of memory from multiple types, invalidating the security guarantee and rendering the approach unsound as stated in Section~\ref{subsec:memorysafetyforheap} and~\ref{subsec:comprehensive}.  
\begin{comment}
\trent{Where do we describe this limitation precisely?  Refer to that text or it needs to be added.} \kaiming{I think the above text (starting from "Some researchers") already described the issue precisely. Basically, the issue is caused by they utilized "allocation-site" instead of "concrete type" for dynamically-typed objects (i.e., the type of the allocation cannot be identified statically), to guide the allocation and reuse memory of such cases. Since per-allocation-site pool may contain multiple types of objects, this causes memory reuse of different types.} 
\end{comment}

\trent{our allocator reqs} Theoretically, \tool needs a memory allocator such that: (1) Heap objects allocated using per-type pool allocation scheme cannot have spatial or type memory errors. (2) The construction of pools should strictly obey per-type design. (3) Heap objects that have spatial or type memory errors should be isolated in a separate region. (4) Memory allocated for a specific type of objects can only be reused later for the same type. Thus, in this paper, we propose runtime enforcement of temporal memory safety defined as type-safe memory reuse~\cite{tat} that overcomes the limitations of prior work to enable efficient protection of heap objects from memory errors comprehensively.


\begin{comment}
TCMalloc~\cite{tcmalloc} is a widely adopted memory allocated and designed to be fast and efficient, it enforces that memory reuse can only be within the same {\em size-class}, but similar to~\cite{tat,tdi}, given multiple types can belong to one size-class, memory reuse across multiple types is still possible. Thus, in this paper, we propose runtime enforcement of temporal memory safety defined as type-safe memory reuse~\cite{tat} that overcomes the limitations of prior work to enable efficient protection of heap objects from memory errors comprehensively.
\end{comment}


\begin{comment}
Theoretically, a sound static analysis that aims for identifying potential temporal safety violations such as UAF and UBI, can be used to fulfill our goal of identifying temporal safe heap objects, we leave that as our future work. 
\end{comment}



%\trent{Separate definition of temporal type safety (and its limitations) from requirements of enforcing that property.  Two separate paragraphs.  For enforcement: Detail or remind of limitations of current typed (or size) pool allocation schemes.  Need to argue we need something new.}

However, the approaches proposed to enforce temporal safety~\cite{cling,tat,tdi,tcmalloc} can suffer from the spatial and type errors that circumvent the type-safe memory reuse guarantee, e.g., overflow can happen within an allocation pool for a specific type.  Enhanced by \tool's static spatial and type safety validation approaches described in Sections~\ref{subsec:spatial} and~\ref{subsec:type}, \tool 
%Given that the objects in the safe region are also validated to be memory safe spatially, 
thwarts the potential threat of violating type-safe memory reuse through spatial and type memory errors, enabling \tool to utilize typed-pool allocation schemes~\cite{safecode,tat} to achieve temporal memory safety. 

\begin{comment}
\trent{Still worried about differentiating from SafeCODE for safety.  Any issues there?} \kaiming{ SafeCode’s type-safe heap reuse design relies on perfect static analysis yielding a complete call graph and precise points-to information, assumptions that are only realistic for small, embedded software~\cite{safecode-gc}. The approach relies on the assumption that static points-to analysis is capable of perfectly determining control flow (including indirect calls) and data flow. Although this may hold for some embedded applications (which are the target of SafeCode), this is unfortunately not the case for complex programs, as DSA has been shown to “lose field sensitivity on up to 70.5\% of tracked struct objects”~\cite{controljujutsu}. Also, they did not provide protection against spatial error exploitations according to their paper~\cite{safecode}, similar to type-after-type, this could result in the bypass of pool allocation. Besides safety concerns, their runtime performance is bad due to the per-function per-type pool design, the goal of having such design is to return memory to the system as soon as possible.}
\end{comment}
%places only objects that pass the type information for statically-proven safe heap objects is available at this stage from the static type validation phase, so 
%\tool %builds upon spatial and type safe to  leverages the typed-pool allocation scheme~ 
%for each type 
%to enforce temporal type safety correctly to ensure comprehensive memory safety for objects in these heap regions. 

Thus, a legitimate and practical solution to retain comprehensive memory safety (see Definition~\ref{def:memorysafety}) 
%\trent{reference its definition here} \kaiming{Added}
is that (1) for the heap objects that are validated to be spatial and type safe (i.e., statically-proven safe - Definition~\ref{def:staticallyprovensafe}), enforcing temporal type safety in an isolated space, called the {\em safe region}) \trent{safe heap?}, (2) for other unsafe heap objects, allocate them into another isolated area (called {\em unsafe region}) and prevent the corruption of such unsafe heap objects from affecting objects in the {\em safe region}.

\begin{comment}
In this work, \tool relies on typed pool allocation to ensure the {\em temporal type safety} through the instrumentation of the memory allocator - TCMalloc. We acknowledge that \tool does not guarantee the comprehensive temporal safety of heap object, but given the exploitation of temporal safety violations always requires the reclaiming of the memory of the different type - type confusion attack, providing the protection that ensures temporal type safety is responsible for mitigating such attack surfaces. Though \tool leaves the possibility for some temporal safety exploitations, such as reusing the memory of the same type, we deem those scenarios are less harmful to the system and we leave providing more fine-grained temporal safety protection as our future work.
\end{comment}


\subsubsection{Temporal Type Safety Requirements}
\label{subsubsec:temporalrequirement}
%\mat{This is implementation?}

\trent{This was largely in a table previously.  Seems appropriate.}
In the design of \tool, we have to ensure that each heap operation satisfies a set of requirements to achieve temporal type safety for the heap objects in the safe region, which are shown in 
Table~\ref{tab:temporalops}.  
%\trent{Summary of requirements} \kaiming{Adjusted the name of Table~\ref{tab:temporalops}}

First, for {\em allocation} operations to ensure objects are only allocated in memory regions for that object's type, \tool maintains a set of per-type free lists instead of a single free list of the raw memory (as in PTMalloc), so that when an allocation request arrives, the allocator can efficiently find free space from the free list of the corresponding type.   
\begin{comment}
\trent{How is this assignment of memory region to type done initially?  Any issues relative to prior work?}  \trent{Should we account for } \kaiming{TCMalloc constructs per-thread cache and per size-class free lists for small objects ($<$ 256 KB). Specifically, TCMalloc divides the small objects into 88 size classes and constructs free lists per each size-class, and allocates heap objects of different size-class into different, isolated spans. For larger heap objects, when the per-thread free list is empty or the requested size is greater than the freed space, TCMalloc enforces a similar design to the per-thread cache - {\em page heap}, the differences are the page heap is used for handling larger objects and it is in memory. Per-size-class design prevents the reuse of memory from previously deallocated heap objects of different size classes, however, in practice, the size-class and type are not interchangeable in C/C++, memory of different types within the same size-class can still be reused. Also, since per size-class design only prevents reuse of memory of different size-class, the unsafe access introduced by spatial and type errors are not protected at all. For Type-after-type, it suffers the issues in my comment above, the allocation site of dynamic-typed objects permits allocating multiple types of objects in one pool.}
\end{comment}

Second, for {\em deallocation} operations to maintain temporal type safety,  \tool updates the per-type free list, so that when a deallocation request arrives, the allocator can free the space of the object and return the memory region to the free list of the corresponding type.  
\begin{comment}
\trent{How determine the type of the object being deallocated?  I assume this is stored somewhere} \kaiming{Yes, it is determined by static analysis and alias analysis, at runtime, we modified the function signature (malloc and free) to read that type information and notify the allocator. Originally the allocator does this in per-size-class way, so it is pretty convenience for us to change it to per-type}\trent{Compare to prior per-type work.  How does this solve their problems?} \kaiming{We basically reuse their schemes here, so no extra gain for us.}
\end{comment}

Third, for {\em reallocation} operations to ensure correct reuse of memory, \tool requests expanding the space is similar to allocation operations and the request of shrinking the space is similar to the deallocation operations.  Also, for reallocation operations that change the original type, which is essentially type casts, we need to ensure the object is deleted from its per-type free list and move it to the unsafe region.  \trent{How do we ensure that all references refer to reallocated memory location?} \kaiming{The reallocation function would take effect on the original stack pointer that points to the heap objects, we identify them by aliasing analysis.}\trent{I mean at runtime.  This is a runtime mechanism.  May be multiple live pointers.} \kaiming{Yes, at runtime, the reallocation is done by the memory allocator, this is invisible to the program, i.e., there is no need for us to enforce the redirection at the program level since the allocator will handle the reference to the reallocated memory location. Maybe use 2 other examples to express this in a more straight-forward way. (1) There are different allocators, switching from one to another does not need program-level change. (2) For a reallocation operation, take ptmalloc as an example, once there is not enough space for the object to be expanded to a certain size, ptmalloc needs to move the object to another place. This process is invisible to the program level and does not need any change to handle that. For TCMalloc, it is the same, since it supports moving objects across spans.}

\begin{table}[ht]
    \centering
	\small
	\begin{tabularx}{8.5cm}{c|X}
	    \toprule
		\multicolumn{2}{c}{\bf\em Requirements of Heap Allocator Operations}\\
		\midrule
		{\bf\em Allocation}&Upon the allocation request of a heap object X of type T, the allocation operation must ensure X is allocated in the free space within the allocation area solely dedicated for type T. \\
	    \midrule
		{\bf\em Deallocation}&Upon the deallocation request of a heap object X of type T, the deallocation operation must ensure the memory allocated for X previously be collected and preserved only for the future (re)allocation request of objects of type T.\\
		\midrule
		{\bf\em Reallocation}&Upon the reallocation request of a heap object X of type T, if the reallocation request works on the same type T (e.g., expanding the array of type T), the reallocation operation must ensure the acquired free space is from the allocation area solely dedicated for type T for expanding the allocation size, or must ensure the released memory be collected and preserved only for the future (re)allocation request of type T for shrinking the allocation size. If the reallocation requests work on changing the original type T, then the object is moved to be allocated into the unsafe region.\\
		\bottomrule
	\end{tabularx}
            \vspace{0.05in}
	\caption{Summary of Requirements for Enforcing Temporal Type Safety}
    \vspace{-0.2in}
	\label{tab:temporalops}
\end{table}



\begin{comment}

As mentioned in Section~\ref{subsec:motivationsec1}, 
In general, previous temporal safety enforcements typically involve significant runtime overhead because of the need for additional metadata and the resulting increase in instruction overhead. Researchers also expressed interest in employing memory allocators for achieving temporal safe memory allocations and management, AFECode~\cite{safecode} first utilized {\em Automatic Pool Allocation} to enforce the temporal safe memory allocation and reuse on the heap, but occurs relatively high overhead since it is still a software-based solution without directly changing the allocator. Other recent works including ~\cite{tat,ffmalloc21usenix,freeguard17ccs,markus20oakland} has been proposed by leveraging allocators to enforce temporal safety, but often trade runtime or memory overhead for safety and fail to provide comprehensive temporal safety protection.

TCMalloc~\cite{tcmalloc} is Google's customized memory allocation implementation for C and C++. It is designed to be fast and efficient, especially for multi-threaded programs. TCMalloc is widely used in Google products such as Chrome due to its high performance. Compared to glibc 2.3 malloc, TCMalloc is faster, which is important because slow memory allocation can cause application writers to create custom free lists, leading to more complexity and higher memory usage. TCMalloc also reduces lock contention for multi-threaded programs, using fine-grained and efficient spinlocks for large objects and virtually no contention for small objects. In comparison, ptmalloc2 uses per-thread arenas to reduce lock contention, but it has a major issue where memory cannot move between arenas, resulting in wasted space. Also, TCMalloc constructs per-thread cache and free lists for small objects ($<$ 256 KB). Specifically, TCMalloc divides the small objects into 88 size classes and constructs free lists per each size-class, and allocates heap objects of different size-class into different, isolated spans. For larger heap objects, when the per-thread free list is empty or the requested size is greater than the freed space, TCMalloc enforces a similar design to the per-thread cache - {\em page heap}, the differences are the page heap is used for handling larger objects and it is in memory.

By examining the TCMalloc design, it becomes clear why it excels in efficiency, particularly for small objects. Additionally, the security community finds its per-size class design attractive, as it prevents the reuse of memory from previously deallocated heap objects of different size classes, aligning with the objective of thwarting temporal error exploitations. Nevertheless, in practice, the size-class and type are not interchangeable in C/C++, as the design of rounding the size of objects to their corresponding size class can result in multiple types being grouped within the same size-class~\cite{tcmalloc}.

Recent research works that utilize TCMalloc for temporal memory safety have highlighted the aforementioned issue~\cite{tat,tdi}. These studies address the problem by adopting a more precise allocation approach that distinguishes allocations based on type or allocation site, rather than size class. For statically identifiable types, the original TCMalloc allocation API is modified to incorporate the {\em type} attribute when allocating and assigning spans. When dealing with statically unidentifiable types, per allocation site is used instead of per type in a similar manner. Consequently, TCMalloc is extended to support per-type or per-allocation-site allocation (and deallocation) of heap objects.
\end{comment}

\subsubsection{Enforcing Typed-Pool Allocation}
\label{subsubsec:poolallocenforce}

\trent{Implementation?  Yes.  And focus first two paragraphs.}
To fulfill the temporal type safety requirements in Section~\ref{subsubsec:temporalrequirement}, introducing new allocation schemes or proposing new memory allocators is the key solution, as attempted in~\cite{tat,cling,tcmalloc}. Unfortunately, these approaches are found to have security flaws, as mentioned in~\ref{subsubsec:temporaloverview}. TCMalloc~\cite{tcmalloc} is a widely adopted memory allocated and designed to be fast and efficient, it enforces that memory reuse can only be within the same {\em size-class}, but similar to~\cite{tat,tdi}, given multiple types can belong to one size-class, memory reuse across multiple types is still possible. Also, TCMalloc has a built-in flaw where newly allocated objects may partially overlap with previously allocated ones, reusing some of their memory in certain scenarios. Although the original TCMalloc documentation~\cite{tcmalloc} did not explicitly acknowledge this issue,~\cite{tdi} identified the problem without proposing a solution. While this flaw does not impact efficiency, it is a significant concern for temporal safety. Also, in the broader concern of comprehensive memory safety, both of them fail to provide the protection of spatial and type safety.

To address the aforementioned problems, we adopt the design principles from Type-After-Type~\cite{tat} that leveraged TCMalloc and incorporate our own improvements to mitigate their security flaws. TCMalloc, also used by Type-After-Type is designed to be fast and efficient, it constructs per-thread cache and free lists for heap objects of each size-class and supports customized free lists, which is friendly for achieving our goal.   

%\trent{Kind of redundant (1st para) and implementation-y (2nd para) so far.  What about SafeCODE?} \kaiming{SAFECode utilized "Automatic Pool Allocation" approach which is not a direct allocator-based solution but rather add an extra software-layer to manage the allocation. It is resource and runtime consuming and has been abandoned by recent researches, recent researches usually directly make changes to the allocator.}

For all the heap objects that passed the static spatial and type safety validation, in case of types that can be statically identified, we follow the approach outlined in~\cite{tat} by expanding the allocation process with an extra attribute - type. This replaces the original allocation pool based on size-class with one based on type. On the other hand, for types that cannot be statically identified (e.g., dynamically typed objects) and heap objects that do not pass the static safety validation, we modify the allocator to ensure that they are allocated into {\em unsafe region} that is completely segregated from all other per-type allocation pools in {\em safe region}. 
%\trent{Do we define the requirements for this segregation anywhere?} \kaiming{No, I just used segregation as the similar word to isolation, we can change it back to isolation. Basically the isolation of safe region and unsafe region relies on ASLR at current stage with the possibility of hardware-assisted approach in the future.} 
We fix the partial overlap issue by enforcing that the allocation always starts from the beginning of the pool (span).   \trent{Implementation issue.  Discussion for the lack of validation for this issue.}
%\trent{Sounds like we always allocate the an object at the beginning of a pool's memory.  Probably not the case.} \kaiming{Actually the first allocation of the pool always start from the beginning of the pool. Originally, due to the allocation scheme, the first allocation of the pool can somehow starting from some offset from the beginning.} 
The challenge is that there is no official documentation about the cause of this issue, we cannot argue that our fix is complete though we have not seen any violation after applying the fix.  
%\trent{Hmm..., so now this partial overlap problem sounds like an implementation issue, bit a conceptual one.  And the fact that we cannot be sure we have a correct fix bodes poorly for stating right before we discuss soundness.} \kaiming{Yes, it is an implementation issue, but we are the first to provide the fix comparing to previous approaches.}
Thus, we ensure temporal type safety of all statically-proven safe heap objects.

\begin{comment}
\subsubsection{Typed-Pool Allocation Soundness}
\label{subsubsec:allocatesound}

\trent{Why is tcmalloc relevant to soundness?  What requirements must be validated to prove soundness?  Need to state these upfront and then prove them.} \kaiming{This paragraph are the remaining from the previous version before we made changes to the temporal safety section. I guess we don't need it currently since this section is pure runtime enforcement, we can seek the opinion from Professor Tan about this.}
\tool utilizes typed-pool allocation by instrumenting TCMalloc for ensuring the temporal type safety of the program, as illustrated in Section~\ref{subsubsec:poolallocenforce}. First, heap objects that fail the static safety validation are placed in a separate isolated allocation unsafe region to prevent them from corrupting safe heap objects. Since the static safety validation overapproximates the unsafe heap objects in terms of spatial and type safety, we claim this allocation process is sound with respect to isolating the safe heap objects from unsafe heap objects. Also, in the enforcement of typed pool allocation in the safe region, we ensure that safe heap objects can only be allocated in the allocation pool with respect to their type, and memory allocated for one type of object will never be reclaimed for objects of different types. Thus, assume the allocation scheme of TCMalloc is sound, \tool's typed pool allocation scheme is sound as well. Implementation issue might exist such as mentioned in~\ref{subsubsec:poolallocenforce}, we claim such issues do not affect the soundness theoretically.
\end{comment}






==> designbackup.tex <==
%In \tool, (i.e., are singletons) (i.e., they are pointers, and type casts of global aliases to reference a heap object using a different type will be detected in Section~\ref{subsec:typevalidate})(initialized and alive throughout the execution)

%and must not be modified through any intended execution (i.e., reallocation), otherwise the global alias is unsafe. Compliant safe global aliases are either (a) singletons, or (b) fields of global objects that only contain singleton pointers. Global aliases that are fields of global objects that contain fields of other types are considered as unsafe, since potential memory errors in other fields may corrupt the alias. \tool marks safe global aliases as read-only once initialized. Thus, safe global aliases are protected from being corrupted through global memory errors. Stack and heap copies of global aliases are analyzed as stack and heap aliases. Note that computing global aliases may suffer from scalability and precision issues for large programs such as Linux Kernel, as noted in~\cite{hybridglobalalias}, given the current approach is sound we left adopting the proposed technique to reason about global aliases in the future.


%The heap object is considered {\em safe} in \tool's static safety validation if itself and all its aliases are spatial and type safe, temporal safety are enforced at runtime (See Section~\ref{subsec:temporal}). 

%



\if 0
\subsection{Identify Required Static Safety Validation}
\label{subsec:validationoverview}

As there is no existing static analysis to validate temporal safety in general for heap objects, temporal safety of heap data is often enforced at runtime.  SAFECode~\cite{safecode} and Type-after-Type~\cite{tat} aim to ensure memory can only be reused for the same data type to avoid type confusion attacks on memory reuse, which is called {\em temporal type safety} in Type-After-Type.  However, SAFECode's enforcement of temporal-type safety is very expensive due to their approach to allocation and the requirement of exact alias information. SAFECode further ignores the impact of spatial safety. In order to accommodate temporal type safety for unsafe objects, Type-after-Type uses object size as the basis of type for objects whose type cannot be identified statically, resulting in memory being used for allocations of different types of the same size, violating type safety.  As a result, memory safety is not ensured for all three classes. 

To resolve this, We observe that a heap object's {\em allocated-type} (See Definition~\ref{def:alloctype}) {\bf must be preserved} for each allocation, which we called {\em temporal allocated-type safety}.  \tool's runtime allocation ensures that memory can be only reused for the heap objects that have the same allocated type (Section~\ref{subsec:temporal}), ensuring uniformity in memory layout. Thus, \tool's static safety validation must validate spatial and type safety statically, determining the allocated type of each heap object, where reuse is only allowed for the allocated-type. 

We note that many heap objects only have accesses that must satisfy both spatial and type safety.  CCured~\cite{ccured} finds that only aliases used in pointer arithmetic operations may violate spatial safety and that only aliases used in type cast operations may violate type safety.  
%They estimated that approximately 90\% of aliases are only used in accesses that must satisfy spatial and type safety.
Thus, to validate spatial and type safety statically for heap objects, we need to find that all accesses using aliases with pointer arithmetic operations satisfy spatial safety (i.e., spatial safety validation) and that all accesses using aliases with type cast operations satisfy type safety (i.e., type safety validation).  Heap objects where all accesses using aliases satisfying spatial and type safety are trivially safe. \tool's identifying of aliases in need validation relies on the soundness of the CCured classifications.
\fi


%requires spatial safety validation. A pointer used in a type cast (i.e., may violate type safety) is classified as T-{\em susp} (stands for type-suspect). As shown in Figure~\ref{fig:arch}, any heap object with zero unsafe aliases is trivially safe and can be placed in the safe heap. Heap objects aliased by S-{\em susp} and/or T-{\em susp} pointers needs further validation. 


%Memory operations that hold the utmost importance are memory read/write, pointer arithmetic, type cast, allocation, deallocation, and reallocation.

%Figure~\ref{fig:syntax} shows the syntax of types and expressions utilized by \tool.  We modified  CCured's syntax to describe how \tool reasons about the heap.  \tool differentiates between two fundamental categories: atomic types, which include scalars and qualified pointers, and structured types.  For reasons detailed in Section~\ref{subsec:typevalidate}, we equate the types ``void" and ``char" with an empty structured type.  Aliases requiring spatial and/or type safety validation are tagged with {\em S-susp} and/or {\em T-susp}, respectively.  From the perspective of memory safety, the expressions that hold the utmost importance are memory read/write, pointer arithmetic, type cast, allocation, deallocation, and reallocation. %The detailed 
%classification generation and propagation 
%typing rules are listed in Figure~\ref{fig:inferrule}. %Note that almost all heap objects may be spatially unsafe by CCured. 


%\tool's safety validation methods require finding all pointers that may-alias each heap object. To do that, 

\begin{comment}
\zhiyun{My understanding is that SVF's pointer analysis is not sound. It can also be very imprecise when analyzing programs with multiple entry points (syscalls or any program that takes multiple rounds of inputs). That's why we developed our own pointer analysis that is much more precise, specifically for multi-entry programs: ``Statically Discovering High-Order Taint Style Vulnerabilities in OS Kernels, CCS 2021''. Probably can cite it and discuss it.} \kaiming{Our pointer alias analysis is not solely based on the SVF pointer alias analysis but is a combination of PDG and SVF. PDG utilizes SVF internally and has already demonstrated its soundness. The soundness of SVF individually, however, is not formally proved in their paper, but we identified that it satisfied the requirements of being sound when dealing with heap objects from a set of papers~\cite{svf,sui2012issta,sui2014tse,sui2016fse,sui2018tse}. Theoretically, SVF is sound for aliasing of the scenario of stack pointers to heap objects. However, implementation-wise, there could be issues that render it to be unsound, which is related to the relative-soundness that we discussed in DataGuard~\cite{dataguard}. Another important reason for us to pick SVF is that it is used in PDG implementation and is compatible with the toolchain. Thanks for the pointer to the paper, I will discuss it in the last paragraph of this subsection.} 
\zhiyun{Thanks for the clarification. I understand your argument that it is by design sound. However, what I am trying to say is that it is, by design, not sound. In fact, any flow-sensitive pointer analysis is, by design, not sound when analyzing multi-entry programs.
To understand this, consider two entry points 1 and 2, we need to consider the results when entry1() is executed before entry2() and vice versa. We also need to consider different sequences of entry1() and entry2() invocations, e.g., 1-2-1-2-1-1-2, to converge to a fixed point. When there are many entry points, it becomes impractical to enumerate all possible sequences of entry-point invocations. My understanding is that SVF tries to be flow-sensitive but it does not really handle multi-entry applications at all (it assumes a single entry only). Also, nginx, httpd, proftpd, and opensshd are can be viewed as multi-entry programs because they essentially run with a giant loop that processes multiple types of requests (each type of request handler can be considered a different entry point). A sound flow-sensitive pointer analysis will need to analyze multiple loop iterations and converge to a fixed point. That said, if you really want to claim design-level soundness, I think we can potentially configure SVF to perform a flow-insensitive pointer analysis, which by design will over-approximate things.} \kaiming{Thanks for pointing the issue out, we were actually not aware of this issue previously. To me "enumerating different sequences entry to examine possible execution sequences or reach a fixed point" is more like a path-sensitivity issue, and in our work, we already run it in a path-insensitive way, that is the reason why our static analysis often overapproximate unsafe operations and need symbolic execution. Also, a key measure of whether an alias analysis work handles heap soundly is whether it handles heap cloning soundly, SVF did so-called lazy heap-cloning but it is still sound. We use SVF for the intra-procedural alias analysis and use PDG to bridge it to inter-procedural in a context-sensitive way. As I mentioned in the last paragraph of this subsection, we probably discuss it in the discussion or related work.}
\zhiyun{I disagree with your assessment that this SVF is sound when analyzing multi-entry programs (I actually talked to the author of SVF, i.e., Prof. Sui, and he agreed that SVF is not designed to handle multi-entry programs so it won't be sound by design). This is a complicated issue and we have actually written a paper on how to perform a sound alias analysis for multi-entry programs (under submission). The first step we took is to give up flow-sensitivity (and I believe SVF is by design flow-sensitivity). Anyway, I agree perhaps the best we can do now is to just acknowledge this issue and discuss it in the discussion section. } \kaiming{Thanks for the clarification and sorry for the confusion by my reply, I actually was not trying to argue that SVF is sound for the multi-entry programs. Again, actually, we were not aware of this issue previously, we identified that SVF did not provide the proof of its soundness formally, proposed and discussed by~\cite{javaheapcloningase,javaheapcloningpldi,Lattner2007MakingCP} , the sound handling of heap cloning is the judgment of whether a heap alias analysis is sound, and we found SVF qualify this requirement from a set of their paper. I guess the major problem seems to be that only requiring sound heap cloning is not enough. It is exciting to know that you already discussed with Prof. Sui about this issue and made improvement to it. In my previous comment-reply, I wanted to say that we only used “pure SVF”  for the intra-procedural alias analysis (is this still a problem for intra-procedural SVF?) and additionally used PDG - which contains a module named parameter-tree, for handling the aliasing queries inter-procedurally - given they already claimed soundness in the PtrSplit paper~\cite{Liu17CCS} “PtrSplit uses a PDG representation that soundly represents pointer data as parameter trees, and tracks pointer bounds for automatic marshaling and unmarshalling without user involvement.”. Also, one of the reasons that we picked SVF is that PDG also used SVF internally so it is compatible with our toolchain. But, might the case that the PDG also did not handle the multi-entry program soundly, I will check with the guy who currently maintains the PDG framework. I agree with your suggestion that we definitely need to discuss this problem in this paper for the soundness concern. At a high level, we are trying to express this paper in a way similar to DataGuard, where a combination of static analysis and runtime enforcement can be utilized to achieve comprehensive protection of heap objects that are verified as memory safe, that said, my opinion is that this problem can also be discussed in the context of relative-soundness.}
\zhiyun{sounds reasonable to me. My understanding is that no alias analysis (if it is flow-sensitive by design) can claim soundness when handling multi-entry programs. I don't think heap cloning or intra-procedural analysis would change anything.}
\zhiyun{I talked to my student working on the sound alias analysis on this. Here is what he said: I agree that flow-sensitive analysis are by design not sound with multi-entry programs. There is Andersen in SVF, which is flow-insensitive by default (which have a chance to be sound against multi-entry programs). However, it depends on the graph that Andersen is applied on. If it is on StaticValueFlowGraph (SVFG), since the graph is flow-sensitive, the analysis will not be sound. If it is performed on PAG (which is not flow-sensitive), it can have a chance to be sound.}\kaiming{Thanks for making the clarification and the input, I will investigate and probably make adjustments to \tool if needed. Definitely, this is something that we would want to discuss in the paper.}
\zhiyun{one more comment from my student: ``And I think heap cloning or the PDG strategy is about context-sensitive (making the analysis more precise), which doesn’t matter to soundness.''} \kaiming{Yes, heap cloning is about context-sensitive, as I mentioned in the next paragraph, "Heap-cloning is proposed in 2004 for facilitating dynamic symbolic execution and context-sensitive heap pointer alias analysis on Java~\cite{javaheapcloningase,javaheapcloningpldi} and has been brought into C/C++ for facilitating the sound context-sensitive heap pointer alias analysis in 2007~\cite{Lattner2007MakingCP}". Alias analyses that aimed to be sound and context-sensitive need to handle heap cloning in a sound way, as discussed in both Sea-DSA~\cite{sea-dsa} and SVF~\cite{Barbar2020FlowSensitiveTH}. Actually the second paper~\cite{Barbar2020FlowSensitiveTH} discussed about combining heap cloning with the flow-sensitive alias analysis and its soundness, and that is the reason why we said it is sound previously as they did not mention the issue that we discussed above. I'm not sure what you mean by "PDG strategy", but the PDG framework introduced by PtrSplit paper~\cite{Liu17CCS} is a sound and context-sensitive pointer alias analysis framework.} 
\end{comment}

\begin{comment}
\kaiming{May put into related work}
SVF heap alias analysis realizes context-sensitive alias analysis on the heap by utilizing the method called {\em heap cloning} soundly. Heap cloning was proposed in 2004 to facilitate dynamic symbolic execution and context-sensitive heap pointer alias analysis on Java~\cite{javaheapcloningase,javaheapcloningpldi} and has been brought into C/C++ for sound context-sensitive heap pointer alias analysis in 2007~\cite{Lattner2007MakingCP}. Heap cloning distinguishes heap objects by (acyclic) call paths, creating copies at the object level, not just by allocation site. Heap cloning is essential because it enables analyses to distinguish different instances of a logical data structure created at different places in a program, even if the data structure is implemented with a common set of functions (e.g., a data structure library) that allocates memory internally. 

While heap cloning itself is sound, SVF aims to perform {\em lazy} heap cloning by incorporating lightweight type information within standard flow-sensitive pointer analysis when applicable~\cite{Barbar2020FlowSensitiveTH}. When an untyped heap object is allocated at a certain point in a program, it can be replaced with a new, uniquely identified object of a specific type, and creates clones based on the type information available at the relevant points in the program. This approach is more efficient since it lazily creates typed objects only at the type initialization points where the object's type is assigned. To retain soundness, SVF requires the program to obey the {\em strict alias rule}, which means dereferencing pointers to objects of different types will never refer to the same memory location. Since our typed-pool allocator 
%based on TCMalloc already 
must satisfy temporal type safety for the safe heap, it must guarantee that no two objects of different types will be placed in the same location by design.
%\trent{Can we assert this requirement up front (for static analysis) and then ensure its enforcement when we discuss runtime.} \kaiming{Yes, we can do it in that way.}
As a result, \tool leverages SVF's heap alias analysis in a sound way. Moreover, given that the PDG representation is claimed to be sound as well~\cite{Liu17CCS}, \tool soundly over-approximates the set of pointers that may alias a heap object.
\end{comment}

%Given the set of aliases, \tool determines which aliases are used in unsafe memory accesses to identify the heap objects requiring further safety validation for the classes of memory that may be violated (i.e., spatial and/or type safety), as described in the next section.  
%Similar to prior work for the stack~\cite{dataguard}, 

\if 0
\begin{figure}
\footnotesize
\begin{gather*}
\begin{aligned}
&Atomic Types: &\alpha ::=\ & \text{int} \mid \tau*\text{Safe}\mid\tau*\text{S-}\textit{susp} \mid \tau*\text{T-}\textit{susp} \mid \tau*\text{Unsafe}\\
&Types: &\tau ::=\ & \alpha \mid \text{void} \mid \text{char} \mid  \tau\{n\} \mid struct\{{\tau_1}{f_1}\ldots{\tau_n}{f_n}\}\\
&Expressions: & e ::=\ & x \mid n \mid \tau(e) \mid e_1+e_2 \mid *e \mid *e_1=e_2 \\
&&&\mid malloc(e) \mid free(e) \mid realloc(e)\\
\end{aligned}
\end{gather*}
\captionsetup{font=footnotesize}
\caption{Programming language syntax of \tool to handle heap alias types, including their validation status (e.g., {\em S-susp} for requiring spatial safety validation), and expressions.}
\label{fig:syntax}
\end{figure}

\begin{figure*}
\scriptsize
\centering
\begin{gather*}
\begin{aligned}
\frac{\Gamma \vdash e_1 : \tau * q \mapsto C_1 \quad \Gamma \vdash e_2 : \text{int} \mapsto C_2}{\Gamma \vdash e_1 + e_2 : \tau * q \mapsto C_1 \cup C_2 \cup \{q = \text{S-}\textit{susp}\}}\ \ \text{(PtrArith)} \quad
\frac{\Gamma \vdash e : \tau_1 *q \mapsto C_1 \quad \Gamma \vdash e : \tau_2 * q \mapsto C_2}{\Gamma \vdash (\tau_2)\ e : \tau_2 * q \mapsto C_1 \cup C_2\cup \{q = \text{T-}\textit{susp}\}}\ \ \text{(Cast)}\quad
\frac{}{\Gamma \vdash (\tau * q)\ 0 : \tau * q \mapsto \emptyset}\ \  \text{(Null)}\quad \quad \quad\\
\\
\frac{\Gamma \vdash e : \tau * q \mapsto C}{\Gamma \vdash (\tau * q)\text{malloc}(e) : \tau * q\mapsto C}\ \  \text{(Alloc)} \quad 
\frac{\Gamma \vdash e : \tau * q \mapsto C}{\Gamma \vdash \text{free}(e) : \tau * q\mapsto \emptyset}\ \  \text{(Free)} \quad
\frac{\Gamma \vdash e_1 : \tau * q \mapsto C_1 \quad \Gamma \vdash e_2 : \tau \mapsto C_2}{\Gamma \vdash (\tau * q)\text{realloc} (e_1, e_2) : \tau * q \mapsto C_1 \cup C_2 }\ \  \text{(Realloc)}\quad\quad\quad\quad\\
\\
\frac{\Gamma \vdash e_1 : \tau * q \mapsto C_1 \quad \Gamma \vdash e_2 : \tau \mapsto C_2}{\Gamma \vdash *e_1 = e_2 : \tau \mapsto C_1 \cup C_2}\ \  \text{(MemWrite)} \quad
\frac{\Gamma \vdash e : \tau * q \mapsto C}{\Gamma \vdash *e : \tau \mapsto C}\ \  \text{(MemRead)} \quad
\frac{}{\tau \ \text{castto int} \mapsto \emptyset} \ \ \text{(ToInt)}\quad
\frac{}{\text{int castto } \tau * q \mapsto \{q = \text{T-}\textit{susp}\}} \ \ \text{(FromInt)}\\
\\
\frac{}{\tau_1 * q_1 \ \text{castto }\tau_2 * q_2 \mapsto \{ q_1 = q_2 = \text{T-}\textit{susp} \lor \tau_1 \approx \tau_2 \} \ \cup \{ q_1 = \text{T-}\textit{susp} \iff q_2 = \text{T-}\textit{susp} \} \ \cup \{ q_2 = \text{S-}\textit{susp} \implies q_1 = \text{S-}\textit{susp} \}} \quad  \text{(PtrCast)} \quad \quad\quad
\end{aligned}
\end{gather*}
\captionsetup{font=footnotesize}
\caption{{\bf \tool Classification Generation and Propagation Type Inference Rule}. Null, Alloc, MemWrite, MemRead, and ToInt rules are similar to CCured, while PtrArith, Cast, FromInt, PtrCast rules are adjusted for heap memory operations. Free and Realloc rules are new.}
\label{fig:inferrule}
\end{figure*}
\fi

%(i.e., to protect temporal safety).  

%Other heap objects require static safety validation to ensure that they can be placed on the safe heap securely. The safety validation required depends on which safety classes are unsafe the aliases of each heap object.  for each memory safety class which their aliases perform unsafe operations.  before they can be placed on the safe heap.  We only validate heap objects for the classes of safety that may be violated.

\if 0
\tool applies the CCured typing judgments as follows:
\vspace{-0.05in}
\begin{itemize}[leftmargin=*]
\setlength\itemsep{-0.2em}
%\item All pointers and objects are classified as \textbf{\em Safe} upon their declaration/allocation.

\item Pointers used in pointer arithmetic operations are classified as \textbf{\em Seq}.  Pointers used in type cast operations are classified as \textbf{\em Wild}.  Otherwise, pointers are classified as \textbf{\em Safe}.  Objects are classified based on the classes of their aliases: \textbf{\em Safe} (i.e., all aliases are \textbf{\em Safe}), \textbf{\em Seq} (i.e., some aliases are \textbf{\em Seq}), \textbf{\em Wild} (i.e., some aliases are \textbf{\em Wild}), or \textbf{\em Seq} $\wedge$ \textbf{\em Wild} (i.e., some aliases are \textbf{\em Seq} and some are \textbf{\em Wild} or some are both).

\item Objects with a \textbf{\em Seq} classification require spatial safety validation as described in Section~\ref{subsubsec:spatialvalidate}. 

\item Objects with a \textbf{\em Wild} classification require type safety validation as described in Section~\ref{subsubsec:typevalidate}. 
\item If objects are not found safe for one or more classes, symbolic validation is applied to remove over-approximations in static analysis as described in Section~\ref{subsubsec:applyse}. 

\item If all \textbf{\em Seq} and \textbf{\em Wild} classifications are found safe, then the object is reclassified as \textbf{\em Safe} and can be deployed on the Safe Heap as described in Section~\ref{subsec:temporal}.  Otherwise, the object is \textbf{\em Unsafe} and is deployed on the regular heap.
\end{itemize}
\fi 

%Upon successful safety validation, such objects are classified back to \textbf{\em Safe}. Upon failure, such objects are classified as \textbf{\em Unsafe} - .

%\item  Upon successful safety validation, such objects are classified back to \textbf{\em Safe}. Upon failure, such objects are classified as \textbf{\em Unsafe} - Section~\ref{subsubsec:typevalidate}.

%\item \textbf{\em Unsafe} objects require symbolic execution validation. Upon success, such objects are classified back to \textbf{\em Safe}. Upon failure, such objects remain \textbf{\em Unsafe} - Section~\ref{subsubsec:applyse}.

\if 0
\vspace{-0.05in}
\subsection{Validate Safety Statically}
\label{subsec:static}

In this section, we detail \tool's static validation methods for spatial and type safety (defined in Section~\ref{subsec:memorysafetyforheap}).  We first describe the static analyses for spatial and type safety validation.  We augment these safety analyses with symbolic execution to remove infeasible aliases that falsely fail validation.  Finally, we summarize the soundness.
\fi



\if 0
Listing~\ref{lst:spatialexample} shows the function {\tt ssl\_asn1\_table\_set} in Apache Httpd Server's SSL module. The function is used to insert or update an ASN.1 SSL private key into a hash table. {\tt asn1->nData} is the original size of the heap object aliased by {\tt asn1->cpData}) defined as constant. At line 5, {\tt length} is declared as the length of the ASN.1 encoded private key. The actual length of the private key can vary, thus, {\tt length} is a non-constant variable. At line 11, the heap object aliased by {\tt asn1->cpData} is dynamically resized through reallocation using {\tt length} if {\tt length} is not equal to {\tt asn1->nData}. The change of the size constraint through reallocation will either not be captured~\cite{ccured,dataguard,safecode}, or treated as an independent new allocation~\cite{duck2018effectivesan,baggybounds,softbound,lowfat,tdi,camp24usenix} in existing works, leaving the original aliases unprotected. In the scenario that multiple aliases access the same object across different threads, if the size is reduced in one thread, then memory accesses from the original aliases in other threads may be rendered unsafe. Thus, bridging the constraints from the object to all its aliases and guaranteeing that all aliases satisfy the current constraint is critical, but remains unsolved.
 %Also, in {\tt else} branch at line 13, {\tt asn1->cpData} is allocated using variable size {\tt length} whose value will be concretized at runtime, static safety validation approaches cannot validate its safety.


\noindent\begin{minipage}{\columnwidth}
\begin{lstlisting}[language=C,caption={Spatial Validation Example},captionpos=b,label={lst:spatialexample}]
ssl_asn1_t *ssl_asn1_table_set(apr_hash_t *table, 
                 const char *key, EVP_PKEY *pkey){
  apr_ssize_t klen = strlen(key);
  ssl_asn1_t *asn1 = apr_hash_get(table, key, klen);
  apr_size_t length = i2d_PrivateKey(pkey, NULL);

  /* Resize if already allocated. */
  if (asn1) {
    if (asn1->nData != length) 
      asn1->cpData = ap_realloc(asn1->cpData, length);
  }
  else {
    asn1 = ap_malloc(sizeof(*asn1));
    asn1->cpData = ap_malloc(length);
    apr_hash_set(table, key, klen, asn1);
  }
  ... // use of asn1->cpData
}

\end{lstlisting}
\end{minipage}
\fi
\if 0
        /* Old version */
      free(asn1->cpData); 
      asn1->cpData = NULL;
      asn1->nData = length;
      if (!asn1->cpData) {
        asn1->cpData = ap_malloc(length);
      }
      /* Old version end */
  else {
    asn1 = ap_malloc(sizeof(*asn1));
    asn1->cpData = ap_malloc(length);
    apr_hash_set(table, key, klen, asn1);
  }
\fi


%Spatial safety validation on heap objects entails four main challenges. First, heap objects can have {\em dynamically-sized} definition \new{(e.g., line 11 in Listing~\ref{lst:spatialexample})}. To handle this case, \new{\tool utilizes value-range analysis to check the {\em size} of the initial allocation must be declared as a constant value, or always bounded by a maximum constant, otherwise the object is flagged as unsafe.}


  \if 0
    \uIf{AllocationSite (alias, object, size)}
    {
        \uIf{$\textit{!(IsConstant(size)) \textbf{or} !(IsConstant(Max(size)))}$}
        {
            $\textit{classify (object, UNSAFE)}$\;
        }
        \Else
        {
            $\textit{size(object)} \gets \textit{size}$ $\textit{   index(alias, object)} \gets 0$\;
        }
    }
    \uElseIf{ReallocationSite (alias, object, newsize)}
    {
        \uIf{$\textit{newsize} < \textit{size(object)}$}
        {
            $\textit{classify (object, UNSAFE)}$\;
        }
        \Else
        {
            $\textit{size(object)} \gets \textit{newsize}$ $\textit{   index(alias, object)} \gets 0$ \;
        }
    }
    
    \Else
    {
    \fi


\if 0
Second, since heap objects are allocated as a unit and represented/accessed as an integrated memory location, it is impractical to enforce field-level isolation within the structure (e.g., as in DataGuard~\cite{dataguard} for stack objects) so \tool reasons about spatial safety at the object (not field) granularity. Thus, if a field in a heap object is accessed unsafely \new{(e.g., {\tt asn1\_cpData} in Listing~\ref{lst:spatialexample})}, \tool classifies the entire heap object as unsafe \new{(e.g., {\tt asn1})}. \tool propagates constraints after converging within a strongly-connected graph of the CFG to reduce resource consumption.  
\fi

%Thus, memory access operations assessed by \tool are with the consideration of multi-threading.

\if 0
Fourth, the declarations of heap objects are determined by their allocation sites, e.g., where {\tt malloc} is called. In some cases, programs create their own allocation wrapper functions \new{(e.g., {\tt ap\_malloc} in Listing~\ref{lst:spatialexample})}, which \tool detects using the technique introduced by Type-After-Type~\cite{tat}.
\fi



% unsafe if field is unsafe (new)
% unsafe if true alias is unsafe (def)
% constraints from allocation functions (allocation)

\if 0
\begin{table}[t!]
    \centering
    \footnotesize
        \scalebox{0.98}{
	\begin{tabularx}{8.5cm}{c|X}
	    \toprule
		\multicolumn{2}{c}{\bf\em Spatial Safety Validation for Heap Objects}\\
		\midrule
		{\bf\em Declaration}&The {\em size} from the object's {\em base}
  must be declared as a constant value, or always bounded by {\em size}.  The initial {\em index} is 0. When {\em size} is changed (i.e., dynamic-size) through realloc to {\em newsize}, {\em newsize} will be recorded for further validation. Reallocations should always increase the size, otherwise, the object is unsafe.\\
	    \midrule
		{\bf\em Definition}& When a pointer is
defined to reference the object, the reference may be {\em offset}
to change the index.  Each safe definition requires this offset to be a constant value.\\
		\midrule
		{\bf\em Use}&When a pointer is used in an
operation, the pointer may be further offset to change the index.  Each safe use requires the offset to be a constant value.\\
		\midrule
		{\bf\em Test}&For all uses, pointer {\em index} 
  $<$ {\em size} and {\em index} $\geq 0$. For dynamic-size, pointer {\em index} 
  $<$ {\em newsize} and {\em index} $\geq 0$.\\	
		\bottomrule
	\end{tabularx}}
        \captionsetup{font=footnotesize}
	\caption{Spatial safety constraints and their use in validation of heap objects}
	\label{tab:spatialconstraint}
 \vspace{-0.3in}
\end{table}
\fi


 

\if 0
\new{Reallocation on shared heap object in multi-threaded programs requires careful and secure management to prevent data corruption or inconsistency. POSIX realloc() employs mutexes internally to protect the memory management metadata to avoid data corruption result in races~\cite{posixrealloc}, however, protecting concurrency issue on dynamically allocated heap data is left at the programmer’s own expertise. Intel suggested programmer adopt thread-safe memory management API~\cite{intelmultithread}, e.g., Intel oneTBB~\cite{intelonetbb}. Meanwhile, allocators~\cite{tcmalloc,ptmalloc,jemalloc} have been designed to leverage thread-local storage/cache and per-thread freelists. Applications such as Nginx and Apache Httpd utilize atomic reallocation operation, they also tend to only use realloc on thread-local data while using alternative data structures (e.g., memory pools and lists) on shared data.}

\new{With these facts above, to deal with reallocation in multi-threaded programs, Uriah relies on the assumption that the reallocation operation is atomic (i.e., memory access operations must not race with reallocation operation). We argue that this assumption is reasonable and aligns with the efforts above. Moreover, Uriah’s static safety validation only allows reallocations that increase the size of the heap object (see Table~\ref{tab:spatialconstraint}), which means the memory access that satisfies the original size constraints should naturally satisfy the new size constraints, memory access that is deemed unsafe stays unsafe and will not be checked again using new size constraints. Thus, our spatial safety validation is valid on the multi-threaded programs that utilize realloc. }
\fi
%Note that we ignore the programmer's intended behavior on performing memory access operations on the original heap object after reallocation, since such an operation is simply unsafe and should not be used.}




%For spatial safety validation, the size of the heap object must be a constant value that can be determined from the parameters passed to the specific allocation function used as described in  {\bf Declaration}.  Then, we detect pointer definitions that may-alias this heap object in {\bf Definitions} through alias analysis.  Any uses of the alias along the computed def-use chains may adjust the spatial state ({\bf Use}), which is then evaluated ({\bf Test}) for compliance with spatial bounds.
%in Table~\ref{tab:spatialconstraint}.

%Second, each heap object has a set of aliases (pointers) that may be defined ({\bf Definition}) to the object and used ({\bf Use}) in memory operations.  Any offsets applied must be constant values for spatial safety validation to succeed (i.e., find the heap object safe).  
\if 0
A challenge in static spatial validation of the heap is that the number of false aliases is much greater for the heap than for the stack, which causes a greater fraction of objects to be classified as unsafe unnecessarily.  %DataGuard ~\cite{dataguard} shows that over 94.9\% of stack objects could be validated as satisfying spatial safety using value-range analysis, but 
\tool finds only 71.7\% of heap objects satisfy spatial safety using this value-range analysis (see column VR in Table~\ref{tab:OverviewEval}).  In Section~\ref{subsec:applyse}, we apply symbolic execution to remove false aliases.


\noindent%\begin{minipage}{\columnwidth}
\begin{lstlisting}[language=C,caption={Spatial Validation Example 1},captionpos=b,label={lst:spatialexample1}]
#define YY_BUF_SIZE 32768
#define YY_CURRENT_BUFFER_LVALUE yyg->yy_buffer_stack[yyg->yy_buffer_stack_top]

static int yy_get_next_buffer (yyscan_t yyscanner) { 
  struct yyguts_t *yyg = (struct yyguts_t*)yyscanner;
  ...
  // # of characters are moved to buffer start.
  int number_to_move = (int)(yyg->yy_c_buf_p 
                    - yyg->yytext_ptr - 1);
  ...
  // Left spaces in buffer after moving
  int num_to_read = YY_CURRENT_BUFFER_LVALUE->
                    yy_buf_size - number_to_move - 1;

  // b is a reference to current buffer
  YY_BUFFER_STATE b = YY_CURRENT_BUFFER_LVALUE;
  ...
  // Reallocate the buffer to accomodate 2 EOB chars.
  b->yy_ch_buf = (char *)ap_expr_yyrealloc(
                    (void *)b->yy_ch_buf, 
                    b->yy_buf_size + 2, yyscanner);
  ...
  // Recalculate # of characters to read.
  // The yy_buf_size is already added by 2.
  num_to_read = YY_CURRENT_BUFFER_LVALUE->yy_buf_size 
                    - number_to_move - 1;
  
  // Read more data into the buffer.
  YY_INPUT((&YY_CURRENT_BUFFER_LVALUE->
                    yy_ch_buf[number_to_move]), 
                    yyg->yy_n_chars, num_to_read);
  ...
}

\end{lstlisting}
%\end{minipage}
\new{Listing~\ref{lst:spatialexample1} shows part of the {\tt yy\_get\_next\_buffer} function used in the expression scanner (httpd/server/util\_expr\_scan.c) of Apache Httpd (2.4.58 - most recent stable version, commit number 339cb1b), designed to manage the dynamic input buffer used during lexical analysis. We simplified the code to remove unnecessary operations and logic. The function manages the input buffer {\tt yyg}, ensuring it's refilled with new data when needed. It shifts unprocessed data to the buffer's start, reallocates the buffer if more space is required, and reads new input into the buffer.}
\new{The size of the input buffer {\tt yyg} is defined as constant initially through a Macro at line 1. The point of interest is in lines 19 - 21. The {\tt yy\_ch\_buf} can be dynamically resized to a greater constant size ({\tt yy\_buf\_size + 2}) to accommodate 2 EOB characters. The access range of the following read operation is updated correspondingly for the new size.}
\new{DataGuard's spatial safety validation is not aware of the dynamic size change of an object. It will validate the memory access based on the size constraints of the initial definition of the buffer size - 32768. The validation will fail since the read operation at line 28-30 will be determined to access out-of-bound memory, which is a mis-classification.}
\new{Given the fact that this code snippet dynamically resizes the input buffer {\tt yyg} using the wrapper {\tt ap\_expr\_yyrealloc}, Uriah's spatial safety validation updates the spatial safety constraints correspondingly using the rule {\em Declaration} in Table~\ref{tab:spatialconstraint} to update the size of {\tt yyg}. Thus, Uriah is able to validate the following read satisfies the spatial safety constraints of {\tt yyg} and classify it as safe.}
\new{DataGuard's spatial safety validation is not aware of the dynamic size change of an object. It will validate the memory access based on the size constraints collected upon the definition of the {\tt asn1->cpData}. Since the size of {\tt asn1->cpdata} is defined as a constant based on the cryptographic algorithm used in the SSL protocol (e.g., 3072 bytes for RSA), DataGuard's spatial safety validation would classify the {\tt asn1} as safe.}
\fi
%\new{Using the spatial safety validation introduced in Algorithm~\ref{algo:spatial}, Uriah is able to validate the example in Listing~\ref{lst:spatialexample}. Given the fact {\tt asn1->cpData} is dynamically resized using the wrapper {\tt ap\_realloc} with non-constant value which can be less than {\tt asn1->nData}, Uriah's spatial safety validation identifies {\tt asn1\_cpData} as unsafe. Thus {\tt asn1} will be flagged as unsafe by Uriah's spatial memory safety validation.}
\if 0
% TJ: redundant with symbolic exec
to accessof each heap object determines their unsafe operations.  However, the set of aliases for each heap object may be over-approximated due to the sound alias analysis approach used by \tool. For the heap, the number of false aliases is much greater than for the stack, causing objects to be classified as unsafe unnecessarily.  
%DataGuard's spatial safety validation for the stack~\cite{dataguard} proved individual objects were safe using a limited scope symbolic execution.  Given the long lifetime of heap objects, such an analysis is impractical.  Instead, 
We find that proving no feasible path for an alias to reference a heap object when unsafe uses occur is an effective way to eliminate false positive aliases. Thus, we require a feasible path from the definition of an alias to the unsafe use of the object, as shown under {\bf Definition}.
%in Table~\ref{tab:spatialconstraint}.  
We describe this feasible path analysis using symbolic execution in Section~\ref{subsubsec:applyse}.
\fi 
\if 0
% TJ: same as before essentially
Third, to determine whether the accesses to a heap object comply with spatial safety, \tool first performs a {\em def-use
  analysis}~\cite{LLVM-def-use} on each unsafe alias, 
%\trent{"pointer detected"?  Aliasing?  Need to specify this.} \kaiming{Seq pointers from CCured and their aliases} 
%LLVM uses SSA form for its
%intermediate representation, so each pointer has only one definition,
%but may have many uses 
as described under {\bf Use} 
%in Table~\ref{tab:spatialconstraint}.  
To assess
bounds statically, \tool performs a {\em value range
  analysis}~\cite{value-range-book,Douglas11SBLP} for
each pointer use from its definition, similar to DataGuard~\cite{dataguard}, to track the range (interval) of pointer arithmetic at each point of a program's execution. We perform a context-sensitive value range analysis to enable the analysis to scale as necessary for heap objects by apply call-strings~\cite{sharir-pnueli} on the PDG.  Soundness is still retained in this approach as we classify any validation that requires exploring beyond the pre-set context-sensitivity level as unsafe. 
\begin{mybox}
    \begin{mythm}
To validate spatial safety, we employ the sound value-range analysis~\cite{value-range-book,Douglas11SBLP,baggybounds}, which is conducted for the def-use chain of all aliases. \tool obtains concrete size constraints, even for resizing. As the collecting aliases and the value-range analysis are sound, \tool's spatial safety validation is also sound.
    \end{mythm}
\end{mybox}
\fi


\if 0
   \uIf{AllocationSite \textbf{or} ReallocationSite}
    {
        \uIf{$\textit{!(IsConcrete(DelayAssignment(alias, object, type)))}$}
        {
            classify (object, UNSAFE)\;
        }
        \uElseIf{ReallocationSite}
        {
             \uIf{$\textit{newsize} < \textit{size(object)}$}
            {
                $\textit{classify (object, UNSAFE)}$\;
            }
        }
        \Else
        {
            ${\textit type(object)} \gets {\textit type}$ ${\textit type(*alias)} \gets {\textit type}$\;
        }
    }
    \Else
    {
\fi



\if 0
\noindent%\begin{minipage}{\columnwidth}
\begin{lstlisting}[language=C,caption={Type Validation Example},captionpos=b,label={lst:typeexample}]
typedef struct {
    ngx_str_t name;
    void      *(*create_conf)(...);
    char      *(*init_conf)(...);
} ngx_core_module_t;

typedef struct {
    ngx_str_t name;
    void      *(*create_conf)(...);
    char      *(*init_conf)(...);
    ngx_event_actions_t     actions;
} ngx_event_module_t;

ngx_cycle_t *
ngx_init_cycle(ngx_cycle_t *old_cycle)
{
    ...
    ngx_core_module_t  *module;
    ...
    for (i = 0; cycle->modules[i]; i++) {
        module = cycle->modules[i]->ctx;
        if (module->create_conf) 
        // create configuration
    }
    ...
}
\end{lstlisting}
%\end{minipage}

\new{Listing~\ref{lst:typeexample} shows {\tt ngx\_init\_cycle} function in Nginx's core module (most recent version 1.25.4). At line 18, {\tt module} is defined as type {\tt ngx\_core\_module\_t*} (definition at line 1). At line 21, {\tt module} is assigned by {\tt cycle->modules[i]->ctx} which is declared as a {\tt void*} pointer and can point to data of different types depending on the specific module type of {\tt cycle->modules[i]}, resulting an implicit typecast from the type of {\tt cycle->modules[i]->ctx} to {\tt ngx\_core\_module\_t}}.
\fi



\if 0
\begin{table}[t!]
    \centering
    \footnotesize
        \scalebox{0.98}{
	\begin{tabularx}{8.5cm}{c|X}
	    \toprule
		\multicolumn{2}{c}{\bf\em Type Safety Validation for Heap Objects}\\
		\midrule
		{\bf\em Declaration}&Heap objects are
assigned the type $\tau$ used in the declaration through allocation functions such as malloc. \\
	    \midrule
		{\bf\em Definition}& When a pointer is
defined to reference the heap object, if the operation includes a type cast
the newtype $\tau^\prime$ is identified. The newtype $\tau^\prime$ is recorded with the original type $\tau$. \\
		\midrule
		{\bf\em Use}&When a pointer is used to
reference the object, if the operation includes a type cast the 
  newtype $\tau^\prime$ is identified.  The newtype $\tau^\prime$ is recorded with the original type $\tau$. \\
		\midrule
		{\bf\em Test}& For a definition or
use that produces a newtype $\tau^\prime$, require that the  newtype $\tau^\prime$ and type $\tau$ are {\em compatible} types.\\
		\bottomrule
	\end{tabularx}}
	\caption{Type safety constraints and their use in validation of heap objects}
	\label{tab:typeconstraint}
 \vspace{-0.3in}
\end{table}
\fi

% problem and goal



%Note that the safety of the uses of the \textit{values} before/after type casts will still be validated by the other static analyses (e.g., access by index will be verified by spatial validation).



%The physical subtyping relation $\tau \ \lesssim \ \tau^\prime$ can be understood as follows: $\tau$ is considered equal to the combination of $\tau^\prime$ and some other lists (which may be empty) of atomic $\tau^{\prime\prime}$. Note $\tau^\prime$ need not be  contained in $\tau$, as long as all the fields of the $\tau^\prime$ are at the same offsets and of the same types in $\tau$, cast from $\tau$ to $\tau^\prime$ ensures that an access at any offset within $\tau^\prime$ references the same type~\cite{ccured-toplas}.
\if 0
\vspace{-0.25in}
\begin{center}
\begin{align}
\tau \ \lesssim& \ \tau^\prime \ \xLeftrightarrow{\text{def}} \exists\ \tau^{\prime\prime}. \ \tau \ \approx \ \tau^\prime\  @ \ \tau^{\prime\prime}.
\end{align}
\end{center}
\vspace{-0.05in}
\fi

\if 0
Moreover, as a relax to the CCured's upcast rule, $\tau^\prime$ is not necessary to be actually contained in $\tau$, as long as all the fields of the $\tau^\prime$ are at the same offsets and of the same types in $\tau$, cast from $\tau$ to $\tau^\prime$ can be deemed as upcast, as follows which is not explicitly captured in prior works~\cite{ccured-realworld,ccured-toplas,hextype,caver,typesan}.
\vspace{-0.25in}
\begin{center}
\begin{align}
\tau\ =&\ \{t_1,\ t_2,\ \ldots,\ t_n,\ t_1^\prime,\ t_2^\prime,\ \ldots,\ t_m^\prime\}\\
\tau^\prime =&\ \{t_1,\ t_2,\ \ldots,\ t_n\}
\end{align}
\end{center}
\vspace{-0.05in}
\fi
%An example of an upcast is shown in Figure~\ref{fig:upcast1}, where where one type (i.e., {\tt tiny\_t}) serves as a field in another type (i.e., {\tt huge\_t}).  Since the beginning of any {\tt huge\_t} structure is a {\tt tiny\_t} structure, a cast of a pointer from {\tt huge\_t} to {\tt tiny\_t} only accesses the object's fields in the expected locations using the same data types, i.e., those defined by the {\tt tiny\_t} type.  


%Figure~\ref{fig:upcast2} shows a second type of upcast not explicitly mentioned in prior works~\cite{ccured-realworld,ccured-toplas,hextype,caver,typesan}.
%In this scenario, all fields of the new type resulting from a type cast (i.e., {\tt tiny\_t}) are also declared to be of the same data types as the original type (i.e., {\tt huge\_t}).  
%\trent{I assume we require the same field names although that seems not to be a requirement.} \kaiming{No we do not require the same field names, if the type and offset match then we say it is the same.}\trent{OK.  That satisfies type safety definition in Section 2.  I guess others may be concerned that the fields have different semantics in different types, but this definition is in the spirit of our use of temporal type safety as well.} 
%Since all the fields of the new type are at the same offsets and of the same types, they satisfy the definition of type safety (see Section~\ref{subsec:memorysafetyforheap}).  Thus, all uses of these aliases will access data of the same type despite the typecast. Note that the safety of the uses of the \textit{values} of these aliasing fields will still be validated by the other static analyses, e.g. if the \texttt{index} fields in the tiny and huge structs in Figure~\ref{fig:upcast2} have distinct value ranges that could allow spatially unsafe access to the object being indexed depending on whether the index value originated in a tiny or huge struct, then this would be flagged as unsafe by the spatial safety analyses even though the upcast itself was considered safe.
% As with temporal type safety, such , but accesses that violate memory safety are not possible. 









%To validate type casts, we must consider all versions of type casting operations in C and C++. 
%C++ has 5 different type cast operations, namely {\em static\_cast}, {\em dynamic\_cast}, {\em reinterpret\_cast}, {\em const\_cast}, and {\em C-style\_cast}. {\em Dynamic\_cast} and {\em const\_cast} do not introduce security concerns~\cite{hextype,caver,typesan} %\trent{Are these independent of upcasts?  Not sure why they introduce no concerns.} \kaiming{Section 2.2 of the Hextype paper has a really nice summary of these 5 types of cast in C++, I omitted them here for the concern of spaces. At high level, dynamic\_cast performs runtime checks upon the type cast by using RTTI, which is heavyweight but is always safe. Real world applications such as Chrome and Firefox prohibits use of dynamic\_cast simply because the overhead is unacceptable if always using it. Instead, they utilized static\_cast and that is the reason why type error still prevails. dynamic\_cast and static\_cast are not independent of upcast/downcast. const\_cast is independent of the upcast/downcast, it is used to remove the const identifier in the type, thus it is orthogonal to the type errors.} 
%and {\em C-style\_cast} is automatically translated to either {\em const\_cast}, {\em static\_cast}, or {\em reinterpret\_cast}~\cite{hextype}. Thus, we focus on validating {\em static\_cast} and {\em reinterpret\_cast} by checking for casts between compatible types. If the type of heap objects cannot be concretized statically, which is the major reason why {\em static\_cast} and {\em reinterpret\_cast} are not as safe as {\em dynamic\_cast}, we classify such objects as unsafe.


%\new{Using the type safety validation introduced in Algorithm~\ref{algo:type} (i.e., TypeCastValidation). \tool can identify {\tt ngx\_event\_module\_t} (and all other module data type) is a subtype of {\tt ngx\_core\_module\_t} since its first three fields are identical with the layout of {\tt ngx\_core\\ \_module\_t}. Thus, the implicit type cast at line 21 is always an upcast (i.e., compatible type cast). Uriah is able to identify that this type cast is always safe in all contexts.}


\if 0
\noindent%\begin{minipage}{\columnwidth}
\begin{lstlisting}[language=C,caption={Type Validation Example},captionpos=b,label={lst:typeexample}]
ngx_uint_t  ngx_mail_max_module;

static char *
ngx_mail_block(ngx_conf_t *cf, 
               ngx_command_t *cmd, void *conf)
{
    ...
    ngx_mail_conf_ctx_t *ctx;
    ...
    /* the main mail context */
    ctx = ngx_pcalloc(cf->pool, 
                        sizeof(ngx_mail_conf_ctx_t));
    ...

    /* Number of the mail modules */
    ngx_mail_max_module = ngx_count_modules(
                        cf->cycle, NGX_MAIL_MODULE);

    /* main_conf context, same in all sub-modules */
    ctx->main_conf = ngx_pcalloc(
                        cf->pool, sizeof(void *) * 
                        ngx_mail_max_module);
    ...
    /* srv_conf context, different in sub-modules */
    ctx->srv_conf = ngx_pcalloc(
                        cf->pool, sizeof(void *) * 
                        ngx_mail_max_module);
    ...
}
\end{lstlisting}
%\end{minipage}

\new{A typical example that illustrates the challenges of type safety validation is the {\em void pointer polymorphism}. Void pointer polymorphism is a commonly used feature in Linux kernel and user-space applications to allow handling data of various types without knowing their specific type at compile time. The example in Listing~\ref{lst:typeexample} shows the {\tt ngx\_mail\_block} function in Nginx Server's mail module (version 1.25.4 - most recent version).}

\new{In this example, the references to the configuration setup are initialized to {\tt void*} at lines 20 and 25. Though the main configurations are always the same in all sub-modules, the server configurations can vary in different sub-modules (line 25). Initialize the pointer ({\tt ctx->srv\_conf}) to the server configuration as {\tt void*} can be dangerous. }
\fi

%Heap objects involved in type casts may be accessed by aliases that may violate type safety (see Section~\ref{subsec:memorysafetyforheap}).  
%Such objects must be accessed consistently with respect to their type, so they are type safe. 
%Our aim is to validate that all aliases of a heap object that have type cast operations must never violate type safety (see Section~\ref{subsec:memorysafetyforheap}).  The challenge is to validate that all such type casts must be type safe, i.e., access the object only at valid locations and with the expected types.  Such an idea was first proposed in an extension of the CCured system~\cite{ccured-toplas,ccured-realworld}, but we extend the idea to include internal structures and provide a complete static type safety validation method for C and C++.
%\trent{Is that true or did ccured propose that too?} \kaiming{Yes, CCured did not propose that in the original paper, CCured-toplas proposed that too, they are the same in two papers and the authors are the same, added the reference.} 
% and apply it to memory safety validation broadly.

% past work does not solve summary

\if 0
The focus on enforcing type safety has been to identify type casts and check that they are safe at runtime~\cite{hextype,caver,ubSAN,vtrust,typesan,duck2018effectivesan}, and most of them focus on C++ only, as described in Section~\ref{sec:motivation}. 
%\trent{Kaiming, is above a correct one-sentence summary?  Do they do static analysis to remove checks?  For which?} \kaiming{The summary is correct, they are all runtime checks on the type cast instructions. The only static analysis that they do is to identify type cast instructions.}  
Past work on memory safety validation for the stack only validated the safety of type casts among integer types, as these are common on the stack~\cite{dataguard}.  However, the heap has many structured types, so we must consider whether type casts among structured types can be validated statically. The overall approach is shown in Table~\ref{tab:typeconstraint}.
\fi 


\if 0
For integer variables, since validating type safety involves checking that values do not change on type casts, the core of type safety validation of integer variables is in the static value range analysis, similar to~\cite{dataguard}. For structural heap objects, the challenge is to assess whether the {\em newtype} and {\em type} for all type casts of all aliases to a heap object are compatible types.  Based on Definition~\ref{def:compatibletype}, we claim that the cast from {\em type} to {\em newtype} must be either (1) a cast between equivalent types or (2) an upcast. The identification of (1) is straightforward, we mainly focus on discussing our methods for (2) below.
\fi


\begin{comment}
\begin{figure}[t]
\centerline{\includegraphics[width=2.15in]{Figures/upcast1.png}}
\vspace{-0.1in}
\caption{In this scenario, {\tt huge\_t} includes {\tt tiny\_t} as its first field.  A type cast from  {\tt huge\_t} to {\tt tiny\_t} satisfies type safety (see Section~\ref{subsec:memorysafetyforheap}) because references using the {\tt tiny\_t} alias will access the same fields. }
\vspace{-0.1in}
\label{fig:upcast1}
\end{figure}

\begin{figure}[t]
\centerline{\includegraphics[width=2.15in]{Figures/upcast2.png}}
\vspace{-0.1in}
\caption{In this scenario, {\tt huge\_t} includes fields of {\tt tiny\_t} as its prefix. A type cast from {\tt huge\_t} to {\tt tiny\_t} satisfies type safety (see Section~\ref{subsec:memorysafetyforheap}) because references using the {\tt tiny\_t} alias will access the same data types at the same locations.}
\vspace{-0.2in}
\label{fig:upcast2}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}
  \begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.35]{Figures/upcast1.png}
    \caption{1st Scenario of Upcast}
    \label{fig:upcast1}
  \end{minipage}%
  \begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[scale=0.35]{Figures/upcast2.png}
    \caption{2nd Scenario of Upcast}
    \label{fig:upcast2}
  \end{minipage}
\end{figure}
\end{comment}

\if 0
CCured proposed that upcasts are type safe.  In general, upcasts between two structured types always fall into one of two categories.  The first category, as shown in Figure~\ref{fig:upcast1}, shows the scenario where one type (i.e., tiny\_t) serves as a field in another type (i.e., huge\_t).  \trent{Was this one not identified by CCured?  If not, what are we adding.  We need to be explicit.} \kaiming{This one was identified by CCured, but there is no available implementation previously of that.}\trent{This is the design section.  We say that we extend the idea of CCured to internal structures, but perhaps that idea was known.  Looks like we add some static safety validation support for C++.  If we only provide an implementation, we need to move along.  Need to know what differs from a design perspective.} %\trent{What is the type cast here?  Why safe?} \kaiming{The cast from huge\_t to tiny\_t is safe, since it is an upcast.} 
The second category, as shown in Figure~\ref{fig:upcast2}, shows a scenario where all fields of the new type resulting from a type cast (i.e., tiny\_t) are also declared to be the fields of the original type (i.e., huge\_t) with respect to their original order starting from the base offset of the object. They are type safe because they do not cause any fields to be interpreted as different types. Thus, all aliases will access data of the same type despite the type cast.  Other type casts are considered unsafe.  

To identify the first scenario, we check for all cast instructions, whether the first field of {\em type} (recursively) is the same as {\em newtype}.  
%\trent{Not clear on this one yet.} \kaiming{Take Figure~\ref{fig:upcast1} as an example, checking whether the first field of huge\_t type is tiny\_t.}  
For the second scenario, assuming {\em newtype} has {\em n} fields, we check for all cast instructions whether the first n fields of {\em type} match all the fields in {\em newtype} with respect to the order and sequence. Note that CCured~\cite{ccured,ccured-realworld,ccured-toplas} claims that among all type casts 63\% are of identical types; for the remaining type casts, 93\% are safe upcasts and 6\% are unsafe downcasts; based on this knowledge, we argue that this approach makes huge improvements on top of previous methods. \gang{What's the improvement exactly, if CCured can deal with safe upcasts already?}\kaiming{CCured just mentioned the upcast in their paper without releasing implementation. Plenty of the following works on runtime type checking did upcast check on C++ only, and we extend it to C. This part is described in Section~\ref{subsec:memorysafetyforheap}}
\fi 



\begin{comment}
\mat{At this stage the policy should be clear along with its intentions/effects. So far, the text is too vague and the policy is not defined with sufficient detail.}
\mat{Before going into how you achieve it (starting next subsection), make sure the policy is crystal clear.}
\mat{Say that your static analysis groups objects into different classes (as you're later referring to these classes without introducing them here)} \kaiming{My sense is the detailed description about the classification policy is given in the text above, but turns out the reader might get drown into the text, we will need to name the unsafe objects find by Uriah, such as Uriah-seq and Uriah-wild to make it clear to readers.}\trent{We need to clear about what must be done (policy), what the challenges are and our insight, and then address the challenges one-by-one.  We need to credit other work that we are building on - erring on over-credit.}  
\end{comment}

\if 0
% TJ: collect for later
\subsubsection{Type Safety Validation Soundness}
\label{subsubsec:typesound} 

\tool validates the type safety of heap objects for two cases: (1) \tool classifies the type casts on integer objects that never change their value as safe~\cite{dataguard}, which relies on the value range analysis that has already been proven sound~\cite{value-range-book} and (2) \tool classifies compatible type casts on objects of structured types as safe. As illustrated in Section~\ref{subsec:type}, our compatible type cast identification method is built on top of the definition of upcast in CCured~\cite{ccured,ccured-realworld,ccured-toplas}, which is demonstrated as sound. 
%Though our current methods of identifying upcast may not be complete (i.e., may have false negatives), w
We classify any heap objects that do not pass the safety validation as unsafe, which means we do not mis-classify any unsafe heap objects as safe. Thus, \tool overapproximates the unsafe type casts of heap objects in the program to retain soundness.
\fi

\if 0
\noindent%\begin{minipage}{\columnwidth}
\begin{lstlisting}[language=C,caption={Symbolic Validation Example},captionpos=b,label={lst:symexecexample}]
static ngx_int_t
ngx_event_process_init(ngx_cycle_t *cycle)
{
    ...
    ngx_uint_t          m;
    ngx_event_module_t  *module;
    ...
    for (m = 0; cycle->modules[m]; m++) {
        if (cycle->modules[m]->type != NGX_EVENT_MODULE){
            continue;
        }
        ...
        module = cycle->modules[m]->ctx;
        ...
    }
}
\end{lstlisting}
%\end{minipage}

\new{Listing~\ref{lst:symexecexample} shows a similar example as in Listing~\ref{lst:typeexample}, but there is a slight difference in the implicit cast at line 13. The type cast can be an unsafe downcast as {\tt module} is defined as of type {\tt ngx\_event\_module\\ \_t} while the type of {\tt cycle->modules[i]->ctx} can be {\tt ngx\_core\_\\ module\_t}. However, the check at line 9 guarantees that such a downcast is infeasible in the execution path that satisfies the check (i.e., infeasible path). Uriah's symbolic validation can remove all the execution paths that reach line 14 that do not satisfy the check at line 9. Thus, this case is verified as safe by Uriah.}
\fi


%False positives of the case (1) are found by detecting infeasible paths. False positives of the case (3) are found by detecting infeasible aliasing. \trent{Did you get these classes of false positives from somewhere else?} \kaiming {false positives are from static analyses. We summarised this to 3 causes previously.} False positives of the case (2) are detected by using symbolic execution to validate safety as proposed in prior work~\cite{dataguard}.

%\tool also adds a new symbolic execution analysis to prove type casts are actually safe (i.e., within a limited execution depth). For the type cast validation, similarly, false positives may occur because (1) infeasible paths and (2) false alias. When performing type safety validation, if the type-cast analysis identifies a heap object as unsafe, it is usually because of either an incompatible type cast or missing type information during static analysis. In the former case, which may contain false positives mentioned above, \tool uses symbolic execution from the allocation of the heap object to the type cast instruction that triggers the alarm. In the latter case, \tool directly classifies such objects as unsafe. This approach helps to verify whether it is a true positive. 








% due to the path-insensitive and over-approximated static analyses. 
%false positive unsafe cases caused by overapproximation of sound static analysis at first, then explore cases where it may be possible to prove compliance, since examining path feasibility reduces the workload that causes path explosion than examining constraint compliance. To prune infeasible paths, \tool symbolically executes each unsafe case from its pointer definition to its unsafe uses following its def-use chain. To prune infeasible aliases, \tool symbolically executes each unsafe alias from its declaration to definitions that involve later unsafe uses to determine whether the alias may be assigned to the heap object. The symbolic execution is conducted using S2E~\cite{s2e}, which reports the existence of a path/alias by issuing the corresponding path constraints. Like prior work, we limit the depth of analysis for detecting infeasible paths and aliases.
%but these cases often can be detected early in the def-use chain.  
%We apply these techniques to prune false unsafe cases for both spatial and type safety.

%by examining whether the def of such an alias can reach the unsafe use.  
%\trent{Correct?} \kaiming{Yes, I added some text to further explain the process. Also, I would like to mention that using SymExec can filter some of the false positive cases but not all of them since we essentially do not have an approach to counting the number of false cases in total. E.g., false positives caused by overapproximation in alias analysis. Otherwise, we would be able to fix them all.} 
  %\gang{From this paragraph it's unclear how the first challenge (long def-use paths) is addressed. How is the symbolic execution here different from the symbolic execution in the previous paper on stack objects?} \kaiming{In Dataguard, we use symbolic execution to explore whether the unsafe cases are compliant with the safety constraint or caused by overapproximation. In Uriah, we add another layer of SE to identify infeasible paths at first, then analyze the compliance of safety constraints. This can filter out infeasible paths that are meaningless to examine. Then for the remaining long def-use chain, we apply execution depth on them.}

%\trent{case of missing type info?  Can symbolic execution help?} \kaiming{The missing type info is caused by either (1) Type metadata being lost/corrupted in LLVM, or (2) it is a dynamically typed object. Symbolic execution can only examine whether there is a feasible path / true alias of the ptr and obj between the def and the unsafe cast, it does not know what exactly the type is. Thus, even if there is a feasible path / exists alias, the type info is still missing. Classifying such cases as safe is dangerous.}

\if 0
% TJ: Is this for implementation?
%Copied from DataGuard paper
A challenge in using symbolic execution is to avoid path explosion.
Since \tool employs symbolic execution on the positive (i.e., presumed
unsafe) cases found by static analysis, we only need to symbolically
execute the program from the allocation of heap objects to its last
unsafe use in its def-use chains, through pointers, which improves \tool's ability to
identify safe cases over pure symbolic execution without static
analysis.  \tool applies LLVM’s loop
simplify and canonicalization
technique to reduce the path
explosion problem introduced by loops, as applied in patch generation
to satisfy safety properties~\cite{huang19oakland}. \tool also
leverages symbolic state merging employed by S2E~\cite{s2e} to
eliminate unnecessary forks when encountering branches, which reduces
the number of paths to explore by orders of
magnitude~\cite{s2e-state-merging}.  To avoid path explosion in long
sequences of def-use chains, we limit the analysis depth.  As
longer def-use chains are more likely to lead to unsafe operations, we
focus on shorter paths.  
\fi

\if 0
\subsection{Safety Validation Soundness}
\label{subsec:sound}


%\trent{collect arguments here.  Gang should check.}

In this section, we assess the soundness\footnote{We use the term {\em soundness} by the static analysis community~\cite{yannis18ecoop}, where a sound analysis over-approximates the program's executions.} of \tool's memory safety validation. Validation must be sound to ensure that no unsafe object can be misclassified as safe.  Similar to DataGuard~\cite{dataguard}, \tool relies on {\em relative soundness}, meaning its static analyses are sound if the techniques it applies and the compositions are sound. 
%This allows for more robust safety validation with over-approximation.
%Soundness must be retained in \tool to ensure identified safe objects do not contain unsafe objects. %that would mistakenly be included in the set of safe objects, which could compromise security.

{\bf Soundness of Analysis Foundations}: \tool employs a context-sensitive heap alias analysis, which consists of two approaches: (1) SVF alias analysis~\cite{svf,sui2012issta,sui2014tse,sui2016fse,sui2018tse} at the intra-procedural level, which utilizes {\em heap cloning}~\cite{Lattner2007MakingCP,javaheapcloningase,javaheapcloningpldi} soundly by incorporating type information within flow-sensitive pointer analysis~\cite{Barbar2020FlowSensitiveTH} and (2) PtrSplit PDG~\cite{Liu17CCS} to represent inter-procedural may-aliases, which uses the parameter-tree mechanism to convey aliases inter-procedurally.  Both are claimed sound.


{\bf Soundness for Static Spatial Safety}:
%To establish the potential index ranges when accessing heap objects
To validate spatial safety, we employ value-range analysis~\cite{value-range-book,Douglas11SBLP,baggybounds,dataguard}. This analysis is conducted using the PDG described above using a sound data-flow analysis~\cite{dataguard}. \tool obtains concrete size constraints, even for resizing.  
%The constraints on pointer declarations and/or definitions, along with concrete size allocations through allocation functions, contribute to this analysis. 
As the PDG and the data-flow analysis are sound, it is evident that \tool's value-range analysis is also sound.

{\bf Soundness for Static Type Safety}: \tool validates the type safety of heap objects 
% TJ: nothing new and don't have room for this...
%for two cases: (1) \tool classifies the type casts on integer objects that never change their value as safe~\cite{dataguard}, which relies on the value-range analysis that has already been proven sound~\cite{value-range-book} and (2) \tool classifies 
for type casts between compatible types.
%on objects of structured types as safe. 
As shown in Section~\ref{subsec:typevalidate}, the compatible-type-cast analysis is built on the sound definition of upcasts in CCured~\cite{ccured-realworld,ccured-toplas}. %\tool also extends CCured's definition to cover more upcast cases. 
Our validation is conservative, requiring the types to match exactly to retain soundness.
%\trent{What about the second case?}
%Though our current methods of identifying upcast may not be complete (i.e., may have false negatives), w


{\bf Soundness of Symbolic Execution}: 
%Path explosion in symbolic execution often means that it is impractical to execute all paths in the program, even with loop canonicalization~\cite{huang19oakland} and symbolic state merging~\cite{s2e-state-merging}. 
\tool employs a depth limit to prevent costly scenarios (e.g., path explosion) in symbolic execution, where any terminated symbolic execution implies that the related heap object is unsafe. %Additionally, when conducting symbolic analyses, there might be a compromise on soundness by utilizing concrete values for certain variables~\cite{SurveySymExec-CSUR18, s2e}. \tool adapted the approach used in~\cite{dataguard}, in the spatial safety analysis, \tool only concretizes variables that hold constant values.
%\gang{If those are already constants, why do you need to concretize them?} \kaiming{Maybe I expressed it in the wrong way, my intention is to say only constant value remains constant, others are symbolic.}
%All other variables are initialized with symbolic values. 
\tool's symbolic verification follows the def-use chains of unsafe aliases from either: (1) a declaration to the definition associated with an unsafe use or (2) a definition to an unsafe use, based on Section~\ref{subsec:applyse}. Thus, all paths that could lead to memory error would be symbolically validated before considering heap object as safe.  %\trent{Different from DataGuard all symexec analyses must be complete before we can remove an infeable case.}

Based on above, \tool overapproximates the unsafe heap objects in the program to retain soundness.



\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/UriahOverview.pdf}
    \vspace{-11pt}\captionsetup{font=footnotesize}\caption{The \tool implementation, consisting of methods to (1) identify the heap objects with aliases requiring validation; (2) validate spatial and type safety statically; and (3) enforce temporal type safety at runtime over spatial/type-safe heap objects}
    \Description{The \tool implementation, consisting of methods to (1) identify the heap objects with aliases requiring validation; (2) validate spatial and type safety statically; and (3) enforce temporal allocated-type safety at runtime over spatial/type-safe heap objects}
    \label{fig:impl}\vspace{-8pt}
\end{figure*}

\fi



%When combined, By satisfying spatial and type safety, the objects may all be co-located in a single heap where all memory accesses will satisfy spatial and type safety between pointer definitions and deallocations.  To ensure 

%As described in Section~\ref{subsec:memorysafetyforheap}, researchers have not yet developed a purely static analysis to validate that all aliases of a heap object are free from temporal errors. Instead, researchers have proposed a variety of runtime methods to prevent pointer use without definition and/or after deallocation~\cite{van2017dangsan,dangnull,caver,safecode,freesentry,safecode-gc, duck2018effectivesan,Nagarakatte2010CETSCE,zhou2022fat,ffmalloc21usenix,freeguard17ccs,markus20oakland}, which incur significant runtime and/or memory overhead.  In practice, however, current methods to exploit temporal memory errors leverage dangling pointers (i.e., pointers with temporal error flaws) to reference memory of a different type, such as to interpret a data value as a pointer.  Thus, researchers have proposed implementing {\em type-safe memory reuse} to enforce {\em temporal type safety}~\cite{cling,tat,tdi}, see Definition~\ref{def:temporalsafety}, which restricts allocations in each memory region to a single data type.  While temporal type safety does not entirely prevent attackers from referencing memory using dangling pointers, it does constrain the attacker by ensuring that any access is to an object of the same type and size, which ensures that spatial errors and type errors are not introduced by allocation.
%\trent{Past work enforces this one.  Ideally, would have defined temporal type safety by now.} \kaiming{My opinion is that we need to put all definitions as earlier as possible and reference them when need. Take this as an example, we will also need to mention temporal type safety in earlier sections, putting definition at here would lead to confusion I guess.}

 
%\trent{Why don't they just determine the type at allocation time and then allocate the object from a region in that free list.  Cost?  Is it that much?} \kaiming{I also had this question previously. Basically, there are 2 reasons, the major reason is that there is no such way to determine the type at runtime for all the objects generally. For polymorphic objects in C++, internal data structure can be used such as vtable. For other objects and objects in C, there is no method to identify the type at runtime. And that is why the runtime type-checking mechanisms have high overhead since they need to record extra metadata for this. Another reason is that they claim that there are not many such cases, but we cannot rely on that. Implementation-wise, they modified the allocation function to add an extra parameter - type or allocation site to facilitate the pool allocation. Delaying type identification to runtime, even if it is possible, could still cause compatibility issues.}\trent{Good info here.  Is this all in the background?} \kaiming{The reason of why runtime type checks are expensive and dynamic infering of type should require metadata is in the background.}                                 
  
%\trent{We have three phrases here: temporal type safe (property), per-type pool allocation (mechanism) and per-type memory reuse (class of mechanisms?).  Do we make these topics and their relationships clear in the backgrround?  They are not very well related here.  We need to tighten this somewhere.  But, first I need to figure out the relationship between type-safe memory reuse and per-type pool allocation.} \kaiming{Per-type pool allocation achieves type-safe memory reuse. so temporal type safety is equivalent of type safe memory reuse. Deleted type safe memory reuse to prevent confusion.}

%\trent{our allocator goals.  safe heap.  Key: All are spatial/type safe.  }
%Instead, 
%\tool provides a memory allocator that ensures that temporal type safety is enforced for each allocation of heap objects that satisfy both spatial and type safety.  \tool achieves this goal by ensuring that: (1) heap objects allocated using a per-type pool allocation scheme cannot have spatial or type memory errors and (2) memory regions can have only a single data type for all allocations. For compatible type casts, the heap object is removed from the original pool and freelist, then added to the new pool and its freelist. \tool provides a per-type pool allocator that allocates objects that are statically-proven safe (Definition~\ref{def:staticallyprovensafe}) in a single {\em safe heap} whose allocation method enforces temporal type safety to enforce comprehensive memory safety (Definition~\ref{def:memorysafety}).  Heap objects that fail either spatial or type safety validation are allocated in a separate unsafe heap, which by virtue of the safety validation, contains no reference to the safe heap, enabling the safe heap to be isolated from the unsafe heap.   
%Heap objects that fail either spatial safety or type safety are alllocat Thus, in this paper, we propose runtime enforcement of temporal memory safety defined as type-safe memory reuse~\cite{tat} that overcomes the limitations of prior work to enable efficient protection of heap objects from memory errors comprehensively.

%\trent{safe heap solution}
%Thus, a legitimate and practical solution to retain comprehensive memory safety (see Definition~\ref{def:memorysafety}) 
%\trent{reference its definition here} \kaiming{Added}
%is that (1) for the heap objects that are validated to be spatial and type safe (i.e., statically-proven safe - Definition~\ref{def:staticallyprovensafe}), enforcing temporal type safety in an isolated space, called the {\em safe region}) \trent{safe heap?} \kaiming{Yes, we call it safe region actually.}\trent{that's the point.  Safe heap is more accurate.  Shouldn't we use that term?}, (2) for other unsafe heap objects, allocate them into another isolated area (called {\em unsafe region}) and prevent the corruption of such unsafe heap objects from affecting objects in the {\em safe region}.
